Centralized Management of a Wifi Mesh for Autonomous Farms

Emerging autonomous farming techniques rely on smart devices such as multi-spectral cameras, collecting fine-grained data, and robots performing tasks such as de-weeding, berry-picking, etc. These techniques require a high throughput network, supporting 10s of Mbps per device at the scale of tens to hundreds of devices in a large farm. We conduct a survey across 12 agronomists to understand these networking requirements of farm workloads and perform extensive measurements of WiFi 6 performance in a farm to identify the challenges in meeting them. Our measurements reveal how network capacity is fundamentally limited in such a setting, with severe degradation in network performance due to crop canopy, and spotlight farm networks as an emerging new problem domain that can benefit from smarter network resource management decisions. To that end, we design Cornet, a network for supporting on-farm applications that comprises: (i) a multi-hop mesh of WiFi routers that uses a strategic combination of 2.4GHz and 5GHz bands as informed by our measurements, and (ii) a centralized traffic engineering (TE) system that uses a novel abstraction of resource units to reason about wireless network capacity and make TE decisions (schedule flows, assign flow rates, and select routes and channels). Our evaluation, using testbeds in a farm and trace-driven simulations, shows how Cornet achieves 1.4 $\times$ higher network utilization and better meets application demands, compared to standard wireless mesh strategies.

==> conclusion.tex <==
\section{Conclusion}

==> eval-old.tex <==
\section{Evaluation}

We use trace-driven simulations to evaluate different aspects of \farmernetes' traffic management engine (\S\ref{sec:trace-eval}). We perform control experiments on real hardware to validate our simulator models (\S\ref{sec:simulator_validate}) and to evaluate the feasibility and overhead of configuring routers over LoRAWAN (\S\ref{sec:impl}). 

\subsection{Trace-driven Simulations} 
\label{sec:trace-eval}

\paragraphb{Simulator} We use our measurements from \S \ref{sec:measurements} to build a simulator for simulating \farmernetes. We fit logarithmic curves on our measurements summarized in figure \ref{fig:distance1} to model throughput over the whole spectrum at any arbitrary distance for different settings and bands. The amount of spectrum needed to send a flow of any arbitrary demand over one link can be calculated from these curves. Multiple routers can be connected through these links to form a mesh network. Next, we model interference based on the same curves. If a router overhears communication between another pair of routers and it is at least as close as the receiver from the sender, the amount of spectrum affected by interference is the same as the amount of spectrum needed to send or receive data at the sender and receiver respectively. But as the distance increases, the proportion of spectrum affected goes down at the same rate as the respective logarithmic curve does. This also indirectly models the throughput degradation with multi-hop: a relay node between the sender and receiver uses 1 share of spectrum listening to the sender, 1 share sending to the next hop, and 1 share affected by interference if the next hop has to forward data ahead. We validate these aspects of the simulator by conducting equivalent real-world experiments as discussed in \S \ref{sec:simulator_validate}. 

The simulator provides abstractions to run real-time and data collection flows. Flows are defined by an under-the-canopy source robot at some location, destination as some gateway router, throughput demand, arrival time, duration, deadline, and data to send for data collection flow. Simulator lets us define scheduling policies, set routes for flows, configure channels for the 2.4 GHz band, and select the first hop AP for under-the-canopy robots.

\paragraphb{Baselines}


\paragraphb{Scenario 1: Small scale Deployment} 

\paragraphb{Scenario 2: Large scale Deployment} 


\paragraphb{Comparison with other routing mechanisms}



\begin{figure*}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat{\includegraphics[width=0.4\textwidth]{figures/realtime_qos.pdf} \label{fig:realtime_qos}}
\subfloat{\includegraphics[width=0.4\textwidth]{figures/non_realtime_data.pdf} \label{fig:non_realtime_data}}
\vspace{-10pt}
\caption{Our heuristics result in better performance for real-time flows and improved throughput of the network.}
\vspace{-10pt}
\label{fig:eval}
\end{figure*}

%\subsection{Daily Workload}

Based on \S \ref{sec:workload}, we consider different kinds of tasks to construct a day's workload. We simulate a square-shaped 174-hectare farm that requires 225 routers placed in a 15 $\times$ 15 grid where each router is 90 meters apart. Routers 6, 7, and 8 in the first-row act as the gateway routers to the edge and are the destination for all flows discussed ahead. The workload is 250 minutes long. There are about 30 daily data collection tasks (e.g. thermal data, sensor data) for which 15 MB per task needs to be collected in the first 200 minutes. There are 8 weekly data collection tasks (e.g. hyperspectral images) for which 500 MB per task needs to be collected in the next two weeks, it is useful to schedule these flows when the network is underutilized. Next, there are 150 real-time tasks (teleoperation, edge-controlled tasks) with demands between 10 and 20 Mbps, duration between 5 and 20 minutes, and flexibility of a few minutes.

We start with the naive strategy of doing no scheduling, picking the nearest AP for the first hop, and picking the shortest path by ETX. This quite obviously results in poor performance for real-time flows as shown in figure \ref{fig:eval} but also the poorest utilization since not delaying non-real-time flows results in real-time flows getting poor throughput and the network sits idle once non-real-time flows are finished. LSTF improves performance for real-time flows as it allocates more resources for them. Picking the shortest paths by congestion results in improved throughput for real-time flows, it also increases network utilization as it discovers longer but congestion-free paths that the shortest path by hops could not. Lastly, the heuristic for picking the first hop AP and assigning APs 2.4 GHz channel in a congestion-aware manner improves the performance slightly by helping alleviate occasional local bottlenecks in the first hop.


\begin{figure*}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat{\includegraphics[width=0.4\textwidth]{figures/interference_distance_2ghz_sim_norm.pdf} \label{fig:interference}}
\subfloat{\includegraphics[width=0.4\textwidth]{figures/hops_norm.pdf} \label{fig:multihop}}
\vspace{-10pt}
\caption{Comparing modeling of interference and multihop in simulator with real-world measurements.}
\vspace{-10pt}
\label{fig:eval}
\end{figure*}


\subsection{Simulator Validation}
\label{sec:simulator_validate}
Our throughput models were already guided by measurements from \S \ref{sec:measurements} but to validate interference modeling and multihop behavior, we conducted some experiments with some Wifi routers on a parking lot's roof and then repeated the same experiments in our simulator to compare trends. In the first experiment, we measure the effect of interference between two sender-receiver pairs as the distance between them increases.  We have two pairs of Linux machines connected over Wifi; where one machine runs iperf server, while other sends udp iperf traffic at full capacity. Both the pairs use different Wifi networks but operate on same channel. We vary the distance between the pairs from 5 meters to 100 meters. The average throughput normalized to the maximum throughput (when pairs operate on different channels) is shown in figure \ref{fig:interference}. The same experiment was repeated in the simulator for 2.4 GHz under the canopy scenario, and the trend is compared in the figure.

Similarly, we connected up to 5 routers serially and placed them apart to form up to 4 hops and measured throughput in each scenario. The same experiment was repeated in the simulator. In both cases the throughput degrades in a similar fashion as shown in figure \ref{fig:multihop}.

\subsection{Implementation Feasibility Overheads} 
\label{sec:impl}


==> heuristics-old.tex <==
\subsection{Traffic Management Algorithm}
\label{sec:heuristics}



We divide our management problem into three parts and discuss different heuristics for them.


\begin{figure*}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat[LSTF schedules 10 Mbps flows at t=0 and 20 Mbps flows at t=10 (Throughput=15.8 Mbps)]{\includegraphics[width=0.32\textwidth]{figures/grid2ghz.pdf} \label{fig:2ghzgrid}}
\subfloat[Selecting nearest AP may overwhelm the AP and make it a bottleneck (Throughput=24.2 Mbps)]{\includegraphics[width=0.32\textwidth]{figures/grid2ghz-nearest.pdf} \label{fig:nearestAP}}
% \subfloat[HTB@end-host]{\includegraphics[width=0.5\textwidth]{figures/4f_htb.pdf} \label{fig:6113}}
\subfloat[Contention Aware AP and Channel selection balances workload across APs and spectrum (Throughput=33.4 Mbps)]{\includegraphics[width=0.32\textwidth]{figures/grid2ghz-lc.pdf} \label{fig:congawareAP}}
\vspace{-10pt}
\caption{Flows from 6 robots in a close locality can bottleneck the first hop, temporal scheduling and congestion aware AP and channel selection can improve throughput. The Hue of circles represents congestion and the color represents the 2.4 GHz channel for the respective AP.}
\label{fig:2ghzbtlnck}
\vspace{-10pt}
\end{figure*}

\subsubsection{\textbf{Temporal Flow Scheduling:} }

The unique temporal flexibility of many applications allows us to use scheduling algorithms to load balance limited network resources in the dimension of time. Since our network is best-effort in principle, all flows with no slack time need to be allocated resources irrespective of the fact that available resources at that point may not be enough. In such cases, real-time flows may get degraded QoS, and data collection flow may not be able to back up the entire data within the stipulated deadline. However, slightly degraded performance may still be useful for the farm. Thus flows with no slack time are allocated resources in a greedy manner immediately, whereas the rest of the flows are ordered by Least Slack Time First (LSTF) and checked for schedulability. It is possible that a flow with the least non-zero slack time may not be schedulable as it causes contention for already scheduled flow but a flow with a higher slack time may be schedulable. Thus a non-zero slack time flow is scheduled greedily if it causes no contention for an already scheduled flow. All flows are rescheduled whenever a scheduler is rerun, therefore it is possible that some flows might be preempted.


\begin{table*}[]
\begin{tabular}{|c|l|l|}
\hline
\textbf{Term}                       & Calculation & \textbf{Definition} \\ \hline
$Spectrum(f, r_{src}, r_{dst})$ &    $r_{src}.spectrum \times \frac{f.demand}{Throughput(Distance(r_{src}, r_{dst}), r_{src}.mode)}$         & Amount of spectrum needed to send flow $f$'s \\ & & entire data from $r_{src}$ to $r_{dst}$ over one hop.                \\ \hline
$Interference(f, r_{src}, r_n)$     & $\frac{Spectrum(f, r_{src}, r_dst)^2}{Spectrum(f, r_{src}, r_n)}$            & Amount of spectrum affected for $r_n$ due to the \\ & & transmission of flow $f$ from neighbouring router                \\ \hline
$Contention(r)$                                &  $\sum_{f \in r.flows} Spectrum(f, r, \_) +  $         & Spectrum required at router $r$ to sustain \\ & $\sum_{r_n \in Neighbours} \sum_{f \in r_n.flows} Interference(f, r_n, r)$ & all flows scheduled on it along with \\ & & interference from flows on 
 neighbouring routers           \\ \hline
\end{tabular}
\end{table*}

\subsubsection{\textbf{Access Point Selection and Channel Allocation:}}

The first resource to be allocated is the Access Point (AP) to connect to for the first hop over the 2.4 GHz interface and channel to be used for this transmission. It's natural to connect with the nearest AP as it may use the least amount of spectrum. However, given the limited amount of bandwidth, even a few flows can overwhelm an AP. Figure \ref{fig:2ghzbtlnck} shows a simple scenario where even scheduling 4 $\times$ 10 Mbps flows on one AP can cause congestion and resultingly poor throughput.  The other choice is to connect with the AP in the range with the least amount of contention, where contention is defined as the amount of spectrum needed to support flows passing through that AP taking into account the interference from neighboring devices. Flows are sorted by their demands and are greedily connected with an AP over a channel that minimizes the function: $Contention(AP) + Spectrum(flow, Robot, AP) + \sum_{r_n \in Neighbours} Contention(r_n) + Interference(flow, Robot, r_n)$ given that $AP.channel = r_n.channel$. In case there is already a flow scheduled on the AP, the value of the channel might be fixed, otherwise minimizing the above function should pick a channel with the least amount of interference from the neighbors. Assigning resources greedily sorted by demand improves spectrum efficiency since high demand flows are assigned to AP nearby thus using less spectrum. Figure \ref{fig:congawareAP} shows a congestion-aware assignment of AP and channels that results in significant improvements in the throughput.


\subsubsection{\textbf{Traffic Engineering:}} 

Since MCFP without flow splitting is an NP-Hard problem, we resort to a greedy strategy to find congestion-aware paths. All flows with no slack time are sorted by their demands and greedily allocated paths on the mesh. Mesh networks typically minimize hop count when finding paths, which have been shown to be inefficient w.r.t spectrum efficiency. ETX is another metric that minimizes the expected number of transactions by penalizing low-quality links. Our naive strategy implements this by only considering the best-quality links i.e. first direct links on all four sides of any router. We then find the shortest path by hop count on this grid. Multiple such paths can exist, therefore, we do randomization here to ensure good load balancing. Since this naive strategy does not account for other flows' traffic or congestion, it performs poorly owing to the incast nature of farm workloads. An optimal path allocation may involve many flows being assigned paths longer than the shortest paths by hop on the mesh. We perform the following graph construction for our grid: all routers are connected to the best-quality links on all sides, while picking the shortest path each node's weight is calculated dynamically by following equation:


\begin{equation}
    \begin{alignat}{2}
        w_r(f) = \max(1, Contention(r) + Spectrum(f,r_{prev}, r)) - 1 \\ + \sum_{r_n \in Neighbours} (max(1, Contention(r_n) \\ + Interference(f,r,r_n) - 1)
    \end{alignat}
\end{equation}

This weight takes into account contention on the respective router and the amount of spectrum needed for flow $f$ to use this router. If there is more than enough capacity to support the flow $f$, then the router has weight 0. The second part of the equation does the same calculation for neighbors of router $r$. Figure \ref{fig:5ghzgrid} shows how this algorithm is able to improve throughput by picking longer paths than the naive strategy of picking shortest path by hop count.

\begin{figure*}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat{\includegraphics[width=0.34\textwidth]{figures/grid5ghzhops.pdf} \label{fig:5ghzhops}}
\subfloat{\includegraphics[width=0.34\textwidth]{figures/grid5ghzlc.pdf} \label{fig:5ghzlc}}
\vspace{-10pt}
\caption{Paths allocated to flows and associated throughput for: \textbf{(a)} Shortest Path by ETX/Hop Count (Throughput = 74.5 Mbps) \textbf{(b)} Shortest Path by Congestion (Throughput = 102.6 Mbps)}
\vspace{-10pt}
\label{fig:5ghzgrid}
\end{figure*}


%\radhika{when explaining routing, maybe mention how ETX (roofnet) tries to capture similar metrics in a decentralized manner, but we can do so in a centralized way. Maybe a footnote that is some thing like ``Decentralized protocols to compute high quality routes (with lower loss rates) in wireless meshes (specifically,~\cite{etx-roofnet, aguayo2004roofnet}) attempt to indirectly capture some of these self-interference effects, but do not quite route around congestion. \farmernetes uses global knowledge to directly and more effectively account for congestion and self-interference when computing routes.''}

==> implementation.tex <==
\section{Implementation}

% \radhika{discusses our setup, system, and implementation-related challenges for real-world deployment. Points here could include: (i) how TE server will communicate with on-filed devices, (ii) how to setup routers etc.}

% \radhika{copy-pasting text from earlier. do we still talk about the LoRA setup?}
% We implement such a set up in \S\ref{sec:impl}.~\footnote{LoRA can support a few tens of Kbps of throughput over a long range of up to 15 kilometers, making it a good fit for exchanging control information for traffic management in \farmernetes. In addition, using out-of-band LoRA for this purpose, as opposed to leveraging the in-band WiFi infrastructure, cleanly decouples the control traffic from the data traffic. }


To support \farmernetes, we need to ensure that Wifi routers provide enough programmability to install routes and switch channels remotely. We use ASUS RT-AC86U updated with Asuswrt Merlin firmware which allows us to be able to perform these operations remotely over SSH. We use these routers to do a small-scale real-world deployment as detailed in \S \ref{sec:real_world}. 

The TE algorithm runs on the edge server and communicates with routers and devices either in-band or out-of-band. Using out-of-band communication mediums like LoRa might be cheaper and more robust against any failures within the Wifi mesh. It will also make remote debugging of the network easier. While, in our setup, we do not use LoRa but manually install routes and channel switching instructions, we were able to install routes and change channels using LoRa when a LoRa receiver was attached to the router. 

==> intro-1.tex <==
\section{Introduction}

Emerging precision agriculture and autonomous farming techniques promise to  reduce farm inputs like fertilizers, increase farm yields, reduce wastage, and improve agricultural sustainability \cite{king2017future, schimmelpfennig2016farm, the_economist_2016, vasisht2017farmbeats, fcc-report}. For example, bulk spraying of agrochemicals (herbicides, pesticides, etc) can be replaced with targeted chemical application or de-bugging of individual affected plants by robots. These techniques rely on smart agricultural equipments such as autonomous tractors, agricultural robots and drones, sensors, and hyperspectral cameras.  Today, the widespread adoption of these techniques is fundamentally limited by the lack of network connectivity on farms~\cite{XXX} for collecting data from and operating these diverse smart devices on farms. The connectivity challenged has been recognized as one of critical importance by the Federal Communications Commission (FCC)~\cite{XXX} and the US Department of Agriculture (USDA)~\cite{XXX}.

This paper asks three important questions in this context: (a) What are the networking requirements for on-farm digital applications? \radhika{discuss concern} (b) What are the unique challenges that inhibit successful on-farm networking? (c) What design choices can we leverage from our understanding of computer networks to improve on-farm networking?  \radhika{todo: will edit this a bit to highlight that our design choices emerge from our observations.}

\vspace{6pt}\noindent\textbf{Requirements for On-farm Applications: } We conducted a survey involving a set of 10 \fixme{?} agronomists spanning two institutions, and extensively reviewed relevant literature from agriculture and robotics communities \cite{bogue2020fruit, kamtikar2021fruitarm, tang2020fruitrecognition, sivakumar2021visualnav, insect_detection} \fixme{more here}. We identify three characteristics of emerging workloads: \textit{(i) Large Data Volumes: } The need to periodically collect small amounts of sensor data in farms (e.g. from soil and weather sensors) is well-studied \cite{vasisht2017farmbeats}. In addition, we realized that sensors such as RGB, thermal and hyperspectral cameras generate 10s to 100s MBs of data per hectare. \textit{(ii) Under-canopy Operation: }Increasingly, many sensors and robots operate \emph{under-canopy}, i.e., are completely surrounded by crops. For example, under-canopy robots are essential for planting cover-crops once the primary crop is close to harvest. \textit{(iii) Real-time Tasks: }More interestingly, workloads for autonomous farms also involve real-time tasks, e.g. autonomously controlled under-canopy robots performing targeted bug spraying, berry-picking, etc. These robots must execute complex planning decisions computed remotely by edge servers (that are typically more powerful than on-field robot devices). The robots must therefore stream rich sensor data at 5-20Mbps from under the canopy to the edge device. 
%Such an edge offload for real-time robot control emerged to be the most popular usecase of farm network in our survey \fixme{?}. 
These workloads emphasize the need for a high throughput network in farms that can support 10s of Mbps of per device even under the crop canopy, as opposed to few tens of Kbps supported by typical farm network options such as LPWAN \fixme{cite}.  



\vspace{6pt}\noindent\textbf{On-farm Measurements: }We conducted the first-of-its kind network measurements across a growing season in a cornfield. Our experiments measure the performance of Wi-Fi 6 at both 2.4 GHz and 5 GHz band under different settings(varying distance, varying height of transmission with respect to the crop canopy, etc) and during different times in the farming season. We chose Wi-Fi because Wi-Fi 6 has been touted as a solution for outdoor connectivity \fixme{cite}. Our experiments for 2.4 GHz and 5 GHz spectrum are also relevant for other emerging rural connectivity solutions such as CBRS (Citizens Band Radio Service) which operates in 3.7 GHz \radhika{discuss}. Our measurements reveal the following challenges and solutions:

\noindent\textit{Challenge 1: Crop Canopy Impact -- }
We find that 5GHz WiFi is unable to work well under-canopy, with the effective throughput degrading to zero beyond a short distance of 40m. In contrast, 2.4GHz WiFi is more robust, sustaining upto \fixme{15 Mbps} of average throughput at a distance of \fixme{80 meters}. We further observed that small spatial variations in device location under the crop canopy can impact network throughput. While one would expect 2.4GHz to be more robust to obstacles, we were surprised by the severity with which the performance of 5GHz (configured to make use of the 160 MHz wide band through channel bonding) degrades under-canopy. For transmissions above the crop canopy, on the other hand, 5GHz fared significantly better than 2.4GHz due to its use of wider channels (and more bandwidth), achieving upto 100 Mbps of throughput at distance of 100 m (2.5 $\times$ higher than 2.4GHz). However, this was still 2 $\times$ lower than the throughput 5GHz could have achieved in the absence of crop canopy! While the timing of the farming season impacted the network throughput (due to difference in moisture content in the crops), the high-level trends were consistent. 

\noindent\textit{Solution 1: Multi-plane Mesh Architecture -- }
The insights from these measurements indicate a unique network design for autonomous farms: a multi-hop mesh of routers placed above canopy (e.g. on poles) that operate on two planes: (i) the 2.4GHz plane, where they talk to the under-canopy devices (e.g. robots) over 2.4GHz channels, and (ii) the 5GHz plane, where the traffic is routed at 5GHz above the canopy across the mesh. So an autonomously operated under-canopy robot or sensor would stream its sensed data over a 2.4GHz channel to one of the routers in its range. The data will then be routed across the mesh of above-canopy routers using 5GHz to the edge servers in near vicinity (farmer's home or some service's parked trucks). We note that this architecture is feasible in farms because farms do not suffer from interference from external sources, unlike typical enterprise settings where WiFi is used. This allows us to use most of the Wi-Fi spectrum. 

\noindent\textit{Challenge 2: Incast -- }Capacity is fundamentally limited by spectrum in such a network, i.e., after a point, a denser deployment of Wi-Fi routers does not increase capacity. In particular, we observe that even a handful \fixme{3-4?} of co-located under-canopy devices transmitting at the same time can overwhelm the 2.4GHz link to a router. Over-provisioning the network by adding more routers cannot help in this case as 2.4.GHz is restricted to using three non-overlapping channels, and neighboring routers operating on the same channel would interfere with one another. Likewise, bottlenecks can quickly emerge in the 5GHz plane due to incast pattern of the workload when multiple on-field devices wish to stream data to the edge servers. Vanilla strategies \fixme{better word} like scheduling flows as and when they are requested and shortest-path load-balanced routing are insufficient to meet the demands of farm workloads, even at a small scale with a handful of devices (with the problem exacerbating with increasing scale of autonomous operations). 


\noindent\textit{Solution 2: Predictability \& Spatio-temportal Scheduling --}We observe that, unlike typical WiFi settings with unpredictable traffic patterns, farm workloads are more controlled and allow room for scheduling (e.g. a real-time remote operation for a robot, once requested, need not be scheduled right-away, but should proceed with minimal interruptions once it has been scheduled.). We can therefore improve the effective network utilization (and throughput) through careful traffic engineering and flow scheduling, driven by flow demands and deadlines. This includes tuning the start times of flows, the routes they take, and the channel allocations in both the 2.4GHz and 5GHz planes. Similar to classical traffic engineering problem in other domains (e.g. WANs and datacenter), we formulate this as a multi-commodity flow problem, but extend it to account for the effects of interference and channel allocation (unique to wireless settings) and temporal scheduling (allowed by the more flexible farm workloads). We use our formulation to design preliminary strategies to improve the performance of farm networks, and identify interesting future directions in this context \fixme{this needs an update}. \fixme{add something on pre-emption} 

\textcolor{red}{Deepak: we need a para on how our scheduling improves results. Also, we probably need a name}

\radhika{We also need to say something about our emulation experiments, perhaps in the list of contributions.}

We summarize our contributions below: 

\noindent $\bullet$ We characterize emerging workloads for autonomous farms, thereby identifying the need for a high throughput network that works well even under crop canopy.

\noindent $\bullet$ We conduct a first-of-its-kind measurement of WiFi performance in farms, which highlights the severe impact of crop canopy on network throughput.

\noindent $\bullet$ Guided by our measurement results, we propose a unique network design for autonomous farms that operates on 2.4GHz under-canopy and 5GHz above canopy. 

\noindent $\bullet$ We identify how bottlenecks can quickly emerge on such a network with limited capacity and incast traffic patterns, and design flow scheduling and traffic engineering techniques to improve network performance. 

We do not claim to provide a perfect solution for enabling high throughput network workloads for autonomous farms. We view our work to be a starting point in this exciting domain, with multiple questions open for future research: e.g. do our observed trends extend to other types of crops (beyond cornfields)? how do other connectivity options (e.g. CBRS) perform under canopy, and would our network design extend to these contexts \fixme{discuss}? how do we deal with variable solar power availability on farms, and extend our scheduler to deal with device mobility? etc. We discuss these questions further in \S\fixme{X}.


\fixme{old text below...}






%Such techniques rely on (a) fine-grained and periodic data collection, e.g. multi-spectral cameras and soil sensors, and (b) individualized actuation by farm robots or drones (e.g. targeted spraying), which often need to be remotely controlled by a human sitting in off-field offices (edge) or via the logic residing in edge servers~\cite{earthsense, cloudrobotics}.





\begin{itemize}
    \item Discuss the need for high throughput network:
    \begin{itemize}
        \item Motivating examples like teleoperation, fruit harvest, bug spraying etc. 
        \item Papers from agronomists: some papers included in surveys.
        \item Discussions/survey with agronomists.
    \end{itemize}
    \item Existing networking solutions for farms do not meet these needs
    \begin{itemize}
        \item Discuss Farmbeats
        \item Wifi 6
    \end{itemize}
    \item We benchmark performance of Wifi 6 in corn field which shows how Wifi's performance degrades in presence of crops:
    \begin{itemize}
        \item 5 GHz is not suitable for under the canopy communication, whereas above canopy range is also only upto 100 meters while giving a decent throughput of 100Mbps.
        \item 2.4GHz is suitable for under canopy communication but it does not have a lot of bandwidth and has only 3 non-overlapping channels.
    \end{itemize}
    \item Our discussions with agronomists and surveys highlight the need for a network capable of providing high throughput real time communication. Further, we also learn that most tasks in such settings have flexibility in deadlines/start times.
    \item Our measurements and surveys help us envision
\end{itemize}

==> intro-2.tex <==
\section{Introduction}

%\radhika{need a better title for the paper....}

Emerging precision agriculture and autonomous farming techniques promise to  reduce farm inputs like fertilizers, increase farm yields, reduce wastage, and improve agricultural sustainability \cite{king2017future, schimmelpfennig2016farm, the_economist_2016, vasisht2017farmbeats, fcc-report}. For example, bulk spraying of agrochemicals (herbicides, pesticides, etc) can be replaced with targeted chemical application or de-bugging of individual affected plants by robots. These techniques rely on smart agricultural equipments such as autonomous robots, drones, sensors, and hyperspectral cameras.  Today, the widespread adoption of these techniques is fundamentally limited by the lack of network connectivity on farms~\cite{usb_report,usda_report} for collecting data from and operating these diverse smart devices. The connectivity challenge has been recognized as one of critical importance by the Federal Communications Commission (FCC) and the US Department of Agriculture (USDA)~\cite{usda_report,fcc-report}.

In this paper, we study the networking requirements for on-farm digital applications, and conduct extensive network  measurements on a farm using WiFi 6 to understand the challenges in meeting these requirements. Armed with this understanding, we design \farmernetes, a unique network architecture for supporting farm applications over WiFi. 

% This paper asks three important questions in this context: (a) What are the networking requirements for on-farm digital applications? (b) What are the unique challenges that inhibit successful on-farm networking? (c) What design choices can we leverage from our understanding of computer networks to improve on-farm networking?  

%\noindent\textbf{Requirements for On-farm Applications: } 
We begin with a survey of 12 agronomists doing cutting-edge research on smart agriculture techniques, and an extensive literature review on such techniques~\cite{bogue2020fruit, kamtikar2021fruitarm, tang2020fruitrecognition, sivakumar2021visualnav, insect_detection, barnes2021opportunities, billingsley2008robotics, rose2021responsible}. 
%We find that these techniques primarily involve two types of tasks: (i) collecting and processing on-field sensor data multiple times a day (with sensors such as RGB, thermal and hyperspectral cameras generating as much as 10s to 100s MBs of data per hectare), and (ii) real-time tasks involving robots performing targeted bug-spraying, berry-picking, etc. These sensors and robots often need to offload compute to edge servers that are typically located in the farmer's office or in service trucks parked at the edge of the field. Edge servers are useful for running complex machine-learning models to control autonomous robots (requiring the robots to stream 5-20Mbps of data to the edge in real-time) and for processing the data collected by on-field sensors. Enabling such edge connectivity imposes multiple challenges on the network infrastructure: (i) Many applications require sensors and robots to operate \emph{under-canopy} (e.g. to monitor plant health, treat targeted crops, etc), where they are completely surrounded by crops, which can degrade network performance. (ii) Multiple on-field devices simultaneously streaming data to the edge creates an incast traffic pattern that can quickly overwhelm network capacity. 
 Our survey and study reveal several interesting characteristics of emerging farm workloads: 
\emph{(i) Large volumes of sensor data:} 
The need to periodically collect small amounts (few KBs) of sensor data in farms (e.g. from soil and weather sensors) is well-studied \cite{vasisht2017farmbeats, shinghal2017wireless, ojha2015wireless}. In addition, sensors such as RGB, thermal and hyperspectral cameras can generate 10s to 100s MBs of data per hectare, that must be collected multiple times a day  (average farm size in the US is 178 hectares~\cite{agcensus}). 
\emph{(ii) Real-time tasks:} Autonomous farming further involves robots performing tasks such as targeted bug spraying, berry-picking, etc. A large farm could have tens of such robots operating simultaneously. 
\emph{(iii) Edge offloading:} Resource-constrained on-field sensors and robots often need to offload compute to edge servers that are typically located few Kilometers away in the farmer's office or in service trucks parked outside the field. Edge servers can run complex machine-learning models to control autonomous robots (requiring each robot to stream 5-20Mbps of data to the edge in real-time) and process the data collected by on-field sensors.  \emph{(iv) Under-canopy operation:} Many applications require sensors and robots to operate under-canopy, where they are completely surrounded by crops. 

The scale (tens of devices), bandwidth requirements (10s of Mbps per device), and operation requirements (range and canopies) of these applications is challenging to meet simultaneously. Typical outdoor networks rely on LPWANs which offer few tens of Kbps throughput per device~\cite{lora}. 
%\deepak{It'd be helpful to add some scale information about robots. 5-20 Mbps sounds, but not when you have five robots. I tried to do that for a couple of the challenges above.}
%\radhika{people not getting why this is interesting -- add back text on typical workloads looked at so far, and LoRAWAN}
%, leading to degraded network performance (as discussed next). 
% \radhika{try to shrink this para: first describe workload and edge. Then mention challenges -- incast and under-canopy} 

%These characteristics emphasize the need for supporting 10s of Mbps per device network throughput in farms, even under the crop canopy, as opposed to few tens of Kbps supported by typical farm network options such as LPWAN \radhika{LoRAWAN?} \fixme{cite}. 
%\deepak{Consider: One challenge with this sentence and also, at other places in the paper is that we talk about `per-device' throughput, but never say how many devices till the eval. As a result, two things happen -- readers find the challenge small (10s of Mbps is doable). At the same time, when people see these numbers come up in eval, they look made-up. We should start talking about scale somewhere in the intro, e.g., consider: The scale (tens of devices), bandwidth requirements (10s of Mbps per device), and operation requirements (range, and canopies) of these applications is challenging to meet simultaneously. Typical outdoor networks rely on LPWANs which offer few tens of Kbps throughput per device. 

%}
% %\radhika{work in progress....}
% %, .  

% % We identify three characteristics of emerging workloads: \textit{(i) Large Data Volumes: } The need to periodically collect small amounts of sensor data in farms (e.g. from soil and weather sensors) is well-studied \cite{vasisht2017farmbeats}. In addition, we realized that sensors such as RGB, thermal and hyperspectral cameras generate 10s to 100s MBs of data per hectare. \textit{(ii) Under-canopy Operation: }Increasingly, many sensors and robots operate \emph{under-canopy}, i.e., are completely surrounded by crops. For example, under-canopy robots are essential for planting cover-crops once the primary crop is close to harvest. \textit{(iii) Real-time Tasks: }More interestingly, workloads for autonomous farms also involve real-time tasks, e.g. autonomously controlled under-canopy robots performing targeted bug spraying, berry-picking, etc. These robots must execute complex planning decisions computed remotely by edge servers (that are typically more powerful than on-field robot devices). The robots must therefore stream rich sensor data at 5-20Mbps from under the canopy to the edge device. 
% % %Such an edge offload for real-time robot control emerged to be the most popular usecase of farm network in our survey \fixme{?}. 
% % These workloads emphasize the need for a high throughput network in farms that can support 10s of Mbps of per device even under the crop canopy, as opposed to few tens of Kbps supported by typical farm network options such as LPWAN \fixme{cite}.  



%\noindent\textbf{On-farm Measurements: } 
Motivated by the above requirements, we next set out to investigate how much network throughput can we expect to achieve in a farm by conducting the first-of-its-kind measurement of network throughput in a 32-hectare corn field. Our experiments measured the performance of WiFi 6 at both 2.4 GHz and 5 GHz bands under different settings (varying distance, varying height of transmission with respect to crop canopy, at different points of times in the growing season, etc). We chose to study WiFi as it is readily and globally available, and is a popular connectivity option for rural farms \cite{ojha2015wireless, ubiquity_2020, ayrstone_productivity_2023} where commercial cellular connectivity is not an option.~\footnote{We discuss the relative advantages of a WiFi-based network over other emerging alternatives such as Citizen Broadband Radio (CBRS) in \S\ref{sec:background}, leaving a more detailed investigation of these alternatives to future work.} Farms provide a unique environment to study WiFi performance -- unlike typical enterprise settings where WiFi is used, farms do not suffer from interference from external sources, thereby allowing the use of most of the WiFi spectrum. However, the network throughput and range can be impacted by the presence of crop canopy.
%We chose Wi-Fi because Wi-Fi 6 has been touted as a solution for outdoor connectivity \fixme{cite}. 
%Our experiments for 2.4 GHz and 5 GHz spectrum are also relevant for other emerging rural connectivity solutions such as CBRS (Citizens Band Radio Service) which operates in 3.7 GHz \radhika{discuss}. 

Our measurements revealed the severe impact of crop canopy on WiFi performance. We found that: (i)  5GHz WiFi is unable to work well under-canopy, with the effective throughput degrading to zero beyond a short distance of 40m! In contrast, 2.4GHz WiFi is more robust, sustaining close to 10 Mbps of average throughput at a distance of 100 meters under-canopy. 
%\deepak{perhaps remove the bandwidth info from first point because a reader may confuse if the change is because of freq or bandwidth}
%We further observed that small spatial variations in device location under the crop canopy can impact network throughput. While one would expect 2.4GHz to be more robust to obstacles, we were surprised by the severity with which the performance of 5GHz (configured to make use of the 160 MHz wide band through channel bonding) degrades under-canopy. 
(ii) For transmissions above the crop canopy, 5GHz fared significantly better than 2.4GHz, 
%due to its use of wider channels (and more bandwidth), 
achieving around 100 Mbps of throughput at a distance of 100m (2.5 $\times$ higher than 2.4GHz). (iii) The above-canopy throughput for 5GHz was still 2 $\times$ lower than what it could have achieved at the same distance in the absence of crop canopy! 
%(iv) The timing of the farming season impacts the network throughput due to differences in crop heights, crop moisture content, and crop volume. Despite these variations, the high-level trends were consistent. 
%\radhika{check: did crop height change across our experiments?}
% \noindent\textit{Challenge 1: Crop Canopy Impact -- }
% We find that 5GHz WiFi is unable to work well under-canopy, with the effective throughput degrading to zero beyond a short distance of 40m. In contrast, 2.4GHz WiFi is more robust, sustaining upto \fixme{15 Mbps} of average throughput at a distance of \fixme{80 meters}. We further observed that small spatial variations in device location under the crop canopy can impact network throughput. While one would expect 2.4GHz to be more robust to obstacles, we were surprised by the severity with which the performance of 5GHz (configured to make use of the 160 MHz wide band through channel bonding) degrades under-canopy. For transmissions above the crop canopy, on the other hand, 5GHz fared significantly better than 2.4GHz due to its use of wider channels (and more bandwidth), achieving upto 100 Mbps of throughput at distance of 100 m (2.5 $\times$ higher than 2.4GHz). However, this was still 2 $\times$ lower than the throughput 5GHz could have achieved in the absence of crop canopy! While the timing of the farming season impacted the network throughput (due to difference in moisture content in the crops), the high-level trends were consistent. 


%We design \farmernetes, a network architecture for supporting farm applications, that incorporates two key elements to address the above challenges. 
We used these observations to guide the design of \farmernetes, our proposed network architecture for supporting farm applications, that incorporates two key elements: 

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/smart_farm.pdf}\vspace{-0.1in}
    \caption{\farmernetes' two-tiered architecture uses 2.4 GHz for transmissions under the crop canopy, and 5GHz above the crop canopy.}\vspace{-0.15in}
    \label{fig:dualplane}
\end{figure}

\paragraphbq{(1) Two-tier Mesh Architecture.} 
The insights from our measurements indicate a clear division of responsibility between the 2.4GHz and the 5GHz bands, resulting in a unique network design for autonomous farms -- a multi-hop mesh of routers placed above canopy (e.g. on poles) that operates in two tiers, as shown in Figure~\ref{fig:dualplane}: (i) 2.4GHz under-canopy, where the routers talk to the under-canopy devices (e.g. robots) over 2.4GHz channels, and (ii) 5GHz above-canopy, where the traffic is routed at 5GHz above the canopy across the mesh. So an autonomously operated under-canopy robot or sensor would stream its sensed data over a 2.4GHz channel to one of the routers in its range. The data will then be routed across the mesh of above-canopy routers to the edge servers using the 5GHz band. ~\footnote{An alternative solution is to eliminate the need for under-canopy transmissions by having under-canopy devices use long antenna attachments that stick above crop canopy. However, such attachments are practically infeasible in farms -- under-canopy robots carrying such antennas will cut through crops (ground footprint of crops is much smaller than surface footprint).} %\radhika{why this is more interesting than standard dual-band WiFi meshes might not be coming across} 

Capacity is fundamentally limited by spectrum in such a wireless mesh -- increasing the density of routers beyond a certain point does not increase network capacity due to interference on the spectrum shared by  overlapping channels. This poses a challenge for both the 2.4GHz tier (that can operate on only three non-overlapping channels) and the 5GHz tier (where routers must operate on the same channel to form a mesh). Even 4-5 co-located under-canopy devices transmitting at the same time can overwhelm the 2.4GHz tier. Likewise, bottlenecks can quickly emerge in the 5GHz tier due to the \emph{incast} resulting from multiple on-field devices simultaneously streaming data to the edge servers. These problems exacerbate with increasing scale of autonomous operations in large farms. This motivates the second element of \farmernetes.


%Deploying such a network requires dealing with questions such as how far should the routers be placed -- our measurements show how the effective throughput degrades with distance, implying that a denser deployment can achieve higher throughput. However, . In other words, capacity is fundamentally limited by spectrum in such a network.  \radhika{replace this with specific challenges in the two tiers (from below)}

%However, capacity is fundamentally limited by spectrum in a wireless network, i.e.,  after a point, a denser deployment of routers does not increase capacity due to interference on shared spectrum.

\paragraphbq{(2) Centralized Traffic Management.} 
%We observe that even a handful \fixme{4-5?} of co-located under-canopy devices transmitting at the same time can overwhelm the 2.4GHz plane. 
%Over-provisioning the network by adding more routers cannot help in this case as 2.4.GHz is restricted to using three non-overlapping channels, and neighboring routers operating on the same channel would interfere with one another. 
%Likewise, bottlenecks can quickly emerge in the 5GHz plane due to the \emph{incast} resulting from multiple on-field devices simultaneously streaming data to the edge servers. 
%Vanilla strategies \fixme{better word} like scheduling flows as and when they are requested and shortest-path load-balanced routing are insufficient to meet the demands of farm workloads, even at a small scale with a handful of devices (with the problem exacerbating with increasing scale of autonomous operations). 
%As discussed above, over-provisioning the network by deploying more routers cannot alleviate such bottlenecks beyond a certain point. 
\farmernetes incorporates centralized traffic management (TM) to alleviate the above bottlenecks and improve network performance. This is facilitated by the observation that, unlike typical WiFi settings with unpredictable traffic patterns, farm workloads are more controlled and allow room for scheduling. For example, a real-time remote operation for a robot, once requested, need not be scheduled right-away, but can be delayed by a few minutes. \farmernetes' TM uses global knowledge of flow demands and deadlines to co-optimize the start times of flows (even pausing and resuming them again, if allowed), the routes they take, and how the WiFi channels are configured. It takes into account the cumulative effects of transmission distance, congestion, and interference when making these decisions. 
%The TM runs at the edge and communicates with the on-field routers and devices using LoRAWAN. 

%Our TM engine leverages insights from traffic engineering in other domains (e.g. WANs and datacenter \fixme{cites}), but extends them to account for the effects of interference and channel allocation (unique to wireless settings) and temporal scheduling (allowed by the more flexible farm workloads). 
% Similar to classical traffic engineering problem in other domains (e.g. WANs and datacenter), we formulate this as a multi-commodity flow problem, but extend it to account for the effects of interference and channel allocation (unique to wireless settings) and temporal scheduling (allowed by the more flexible farm workloads). We use our formulation to design preliminary strategies to improve the performance of farm networks, and identify interesting future directions in this context \fixme{this needs an update}. \fixme{add something on pre-emption} 

%We build a simulator to simulate the \farmernetes network architecture, and use it to evaluate the significance of different elements (decision knobs) in its traffic management unit. Our simulator draws upon our on-farm measurements to model per-link throughput. It also models the effect of interference and multi-hop performance, that are backed by measurements on real hardware. 

%\textcolor{red}{Deepak: we need a para on how our scheduling improves results. Also, we probably need a name}

%\radhika{We also need to say something about our emulation experiments, perhaps in the list of contributions.}


We build a simulator to simulate the \farmernetes network and to evaluate its traffic manager. We use our on-field measurement traces and control experiments on real hardware (\S\ref{sec:impl}) to guide the models used in our simulator. Our evaluation show how \farmernetes' TM results in upto 2.5 $\times$ better network utilization and  4 $\times$ better performance for real-time tasks (in terms of throughput normalized by flow demand) when compared with standard wireless mesh strategies. 

We summarize our contributions below: 

\noindent $\bullet$ We conduct the first-of-its-kind measurements of WiFi throughput in a cornfield. 

\noindent $\bullet$ Guided by these measurements, we design \farmernetes, a two-tiered network for autonomous farms. 

\noindent $\bullet$ We design a centralized traffic management engine as part of \farmernetes to improve network performance. 

\noindent $\bullet$ We build a trace-driven simulator (informed by experiments on real hardware) to evaluate \farmernetes. 
%Our evaluation highlight the importance of \farmernetes' centralized traffic management decisions. \radhika{revisit}
We will open-source our measurement traces and our simulator. 

This work does not raise any ethical concerns. 
%\ammar{update as needed}
%\deepak{Should we commit to releasing our measurements and code? People like that.}
% We summarize our contributions below: 

% \noindent $\bullet$ We conduct a survey and literature review to characterize emerging workloads for autonomous farms, identifying the need for a high throughput network that works well even under crop canopy (\S\ref{sec:workload}).

% \noindent $\bullet$ We conduct a first-of-its-kind measurement of WiFi performance in a farm, which highlights the severe impact of crop canopy on network throughput (\S\ref{sec:measurements}).

% \noindent $\bullet$ Guided by our measurements, we design \farmernetes, a unique two-tier network architecture for farms that operates on 2.4GHz under-canopy and 5GHz above canopy (\S\ref{sec:dual-plane}) 

% \noindent $\bullet$ We identify how bottlenecks can quickly emerge on such a network with limited capacity and incast traffic patterns, and design a centralized traffic management engine as part of \farmernetes to improve network performance (\S\ref{sec:te}).  

% \noindent $\bullet$ We build a simulator to simulate the \farmernetes network and to evaluate the significance of different elements (decision knobs) in its traffic management engine. We use our on-field measurements and control experiments on real hardware (\S\ref{sec:impl}) to guide the models used in our simulator. 

%The simulator models per-link throughput based on our on-farm measurements.  We further use control experiments on real hardware to guide our simulator models for interference and multi-hop performance, and to validate the feasibility of implementing some of the proposed techniques (\S\ref{sec:impl}). 

%We do not claim to provide a perfect solution for enabling high throughput network workloads for autonomous farms. We view our work to be a starting point in this exciting domain, with multiple questions open for future research: e.g. do our observed trends extend to other types of crops (beyond cornfields)? how do other connectivity options (e.g. CBRS) perform under canopy, and would our design insights extend to these contexts? how do we deal with variable solar power availability on farms? etc. We discuss these questions further in \S\ref{sec:discussion} \radhika{revisit}.


%\fixme{old text below...}






%Such techniques rely on (a) fine-grained and periodic data collection, e.g. multi-spectral cameras and soil sensors, and (b) individualized actuation by farm robots or drones (e.g. targeted spraying), which often need to be remotely controlled by a human sitting in off-field offices (edge) or via the logic residing in edge servers~\cite{earthsense, cloudrobotics}.





% \begin{itemize}
%     \item Discuss the need for high throughput network:
%     \begin{itemize}
%         \item Motivating examples like teleoperation, fruit harvest, bug spraying etc. 
%         \item Papers from agronomists: some papers included in surveys.
%         \item Discussions/survey with agronomists.
%     \end{itemize}
%     \item Existing networking solutions for farms do not meet these needs
%     \begin{itemize}
%         \item Discuss Farmbeats
%         \item Wifi 6
%     \end{itemize}
%     \item We benchmark performance of Wifi 6 in corn field which shows how Wifi's performance degrades in presence of crops:
%     \begin{itemize}
%         \item 5 GHz is not suitable for under the canopy communication, whereas above canopy range is also only upto 100 meters while giving a decent throughput of 100Mbps.
%         \item 2.4GHz is suitable for under canopy communication but it does not have a lot of bandwidth and has only 3 non-overlapping channels.
%     \end{itemize}
%     \item Our discussions with agronomists and surveys highlight the need for a network capable of providing high throughput real time communication. Further, we also learn that most tasks in such settings have flexibility in deadlines/start times.
%     \item Our measurements and surveys help us envision
% \end{itemize}

%\section{Ethical Concerns}


==> intro-3.tex <==
% Emerging and recent innovations in agriculture like precision agriculture and automation aim to solve critical issues facing the agriculture sector to meet the production demand to feed the growing world population. These challenges include coping with labor shortages and scaling up yield by developing more sustainable agricultural practices and reducing wastage. 
\ammar{I think we can make this start stronger}
Emerging precision agriculture and autonomous farming techniques promise  to meet the critical goals of increasing farm yields, reducing wastage, and improving agricultural sustainability~\cite{king2017future, schimmelpfennig2016farm, the_economist_2016, vasisht2017farmbeats, fcc-report}. 
%, thereby tackling critical global issues such as farm labor shortages and meeting growing food demands
%\ammar{This can be made stronger i.e. showing why supporting these applications is critical for ag sector.}. 
For example, bulk spraying of pesticides can be replaced with targeted chemical application at individual affected plants by robots. 
These techniques rely on smart devices such as autonomous robots, drones, and sensors such as hyperspectral cameras, that require high bandwidth network connectivity for remote operation and data transmission. The widespread adoption of these techniques is fundamentally limited today by the lack of suitable network connectivity on farms. This connectivity challenge has been recognized as one of critical importance by the Federal Communications Commission (FCC) and the US Department of Agriculture (USDA)~\cite{usda_report,fcc-report}. 

%Today, the widespread adoption of these techniques is fundamentally limited by the lack of network connectivity on farms~\cite{usb_report,usda_report} for collecting data from and operating these diverse smart devices. The connectivity challenge has been recognized as one of critical importance by the Federal Communications Commission (FCC) and the US Department of Agriculture (USDA)~\cite{usda_report,fcc-report}.


In this paper, we study the networking requirements for emerging on-farm applications, and conduct extensive network  measurements on a farm using WiFi 6 to understand the unique challenges in meeting these requirements. Guided by this understanding, we design \farmernetes, a WiFi mesh network for farm applications, that incorporates a centralized traffic manager, tailored to the distinguishing characteristics of farm workloads and wireless network, for extracting maximal network performance under challenging conditions. 

%This paper asks three important questions in this context: (a) What are the networking requirements for on-farm digital applications? (b) What are the unique challenges that inhibit successful on-farm networking? (c) What design choices can we leverage from decades of research on network resource management to improve on-farm networking?  \radhika{this needs to be fixed} \ammar{yes, we can make it short by saying that we identify characteristics of these workloads and based on measurements, we build a resource management framework to support these applications with limited network resources available in farms.}

%\ammar{Following paragraph can be made much shorter by just highlighting two things: high throughput applications and flexibility in scheduling such tasks. Maybe survey can be left for next section.}
%\noindent\textbf{Requirements for On-farm Applications: } 
We begin with a survey of 12 agronomists and an extensive literature review to understand the requirements of farm applications. \ammar{Some details here can be omitted, we should instead emphasize on high throughput and flexibility of workload.} \radhika{need some details about scale earlier on} Our study, detailed in \S\ref{sec:workload}, highlights the need for a high bandwidth network to support tens to hundreds of devices that include: (i) sensors transmitting large amounts of data to edge servers located in the farmers home/office a few Kilometers away (e.g. RGB, thermal and hyperspectral cameras that can generate 10s to 100s of MBs of data per acre, with a typical farm spanning a few hundred acres \fixme{cite}), and (ii) robots performing targeted bug-spraying, berry-picking, etc, that are remotely controlled by edge servers, with each device requiring a steady upstream of 5-20Mbps. In many cases, these devices must operate from under the crop canopy where they are completely surrounded by crops. 

%Evidently, the bandwidth requirements of these applications cannot be met using typical outdoor networks based on LPWANs~\cite{lora, chakraborty2022whisper}, which can offer only a few tens of Kbps throughput per device. 
%\noindent\textbf{On-farm Measurements: } 
%Motivated by the above requirements, 
%we next set out to conduct a first-of-its-kind WiFi throughput measurement in an 80 acre corn fiel
%  by conducting the 
%\ammar{Can be made shorter by just saying Wifi despite its short range, allows for high throughput suitable for our workloads and is readily available unlike cellular networks.}  
%Keeping the higher bandwidth requirements in mind, 
Keeping by the above requirements in mind, we next set out to investigate how much network throughput can we expect to achieve in a farm. For this, we conduct a first-of-its-kind network throughput measurement for WiFi 6 (at both 2.4 GHz and 5 GHz bands) in an 80 acre corn field under different settings (varying distance, varying height of transmission with respect to crop canopy, etc).~\footnote{Our reasons for choosing WiFi, detailed in \S\ref{sec:background}, include its relatively higher bandwidth, its ready availability and its popularity (especially in rural farms \cite{ojha2015wireless, ubiquity_2020, ayrstone_productivity_2023} where commercial cellular connectivity is not an option).} 
%~\footnote{We discuss the relative advantages of a WiFi-based network over other emerging alternatives such as Citizen Broadband Radio (CBRS) in \S\ref{sec:background}, leaving a more detailed investigation of these alternatives to future work.} 
%We conduct 
%Farms provide a unique environment to study WiFi performance -- unlike typical enterprise settings where WiFi is used, farms do not suffer from interference from external sources, thereby allowing the use of most of the WiFi spectrum. However, the network throughput and range can be impacted by the presence of crop canopy. \ammar{can be removed or shortened.} 
%We chose Wi-Fi because Wi-Fi 6 has been touted as a solution for outdoor connectivity \fixme{cite}. 
%Our experiments for 2.4 GHz and 5 GHz spectrum are also relevant for other emerging rural connectivity solutions such as CBRS (Citizens Band Radio Service) which operates in 3.7 GHz \radhika{discuss}. 
Our measurements revealed the severe impact of crop canopy on WiFi performance. We found that: (i) 5GHz WiFi is unable to work well under-canopy, with the effective throughput degrading to zero beyond a short distance of 40m! In contrast, 2.4GHz WiFi is more robust, sustaining close to 10 Mbps of average throughput even at a distance of 100 meters under-canopy. 
%\deepak{perhaps remove the bandwidth info from first point because a reader may confuse if the change is because of freq or bandwidth}
%We further observed that small spatial variations in device location under the crop canopy can impact network throughput. While one would expect 2.4GHz to be more robust to obstacles, we were surprised by the severity with which the performance of 5GHz (configured to make use of the 160 MHz wide band through channel bonding) degrades under-canopy. 
(ii) For transmissions above the crop canopy, 5GHz fared significantly better than 2.4GHz, 
%due to its use of wider channels (and more bandwidth), 
achieving around 100 Mbps of throughput at a distance of 100m (2.5 $\times$ higher than 2.4GHz). \radhika{do these numbers need an update?} \ammar{yes, slight updates, will do}
%(iv) The timing of the farming season impacts the network throughput due to differences in crop heights, crop moisture content, and crop volume. Despite these variations, the high-level trends were consistent. 
%\radhika{check: did crop height change across our experiments?}
% \noindent\textit{Challenge 1: Crop Canopy Impact -- }
% We find that 5GHz WiFi is unable to work well under-canopy, with the effective throughput degrading to zero beyond a short distance of 40m. In contrast, 2.4GHz WiFi is more robust, sustaining upto \fixme{15 Mbps} of average throughput at a distance of \fixme{80 meters}. We further observed that small spatial variations in device location under the crop canopy can impact network throughput. While one would expect 2.4GHz to be more robust to obstacles, we were surprised by the severity with which the performance of 5GHz (configured to make use of the 160 MHz wide band through channel bonding) degrades under-canopy. For transmissions above the crop canopy, on the other hand, 5GHz fared significantly better than 2.4GHz due to its use of wider channels (and more bandwidth), achieving upto 100 Mbps of throughput at distance of 100 m (2.5 $\times$ higher than 2.4GHz). However, this was still 2 $\times$ lower than the throughput 5GHz could have achieved in the absence of crop canopy! While the timing of the farming season impacted the network throughput (due to difference in moisture content in the crops), the high-level trends were consistent. 

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/smart_farm.pdf}\vspace{-0.1in}
    \caption{\farmernetes' two-tiered architecture uses 2.4 GHz for transmissions under the crop canopy, and 5GHz above the crop canopy.}\vspace{-0.15in}
    \label{fig:dualplane}
\end{figure}
%We design \farmernetes, a network architecture for supporting farm applications, that incorporates two key elements to address the above challenges. 
%\paragraphbq{\farmernetes' Two-tier Mesh Architecture.} 
%\radhika{the term \farmernetes has not been introduced before}
The insights from our measurements result in a unique WiFi network design for autonomous farms -- a multi-hop mesh of routers placed above the crop canopy (e.g. on poles) that operates in two tiers, as shown in Figure~\ref{fig:dualplane}: (i) \emph{2.4GHz under-canopy tier}, where the routers talk to the under-canopy devices (e.g. robots and sensors) over 2.4GHz channels, and (ii) \emph{5GHz above-canopy tier}, where the traffic is routed to the edge servers across the mesh using the 5GHz band. 
%So an autonomously operated under-canopy robot or sensor would stream its sensed data over a 2.4GHz channel to one of the routers in its range. The data will then be routed across the mesh of above-canopy routers to the edge servers using the 5GHz band. 
~\footnote{An alternative solution is to eliminate the need for under-canopy transmissions by having under-canopy devices use long antenna attachments that stick above crop canopy. However, such attachments are practically infeasible in farms -- under-canopy robots carrying such antennas will cut through crops (ground footprint of crops is much smaller than surface footprint).}

We next come to the challenge of supporting on-farm applications on such a wireless mesh network. This involves supporting tens to hundreds of devices, where each device requires tens of Mbps of bandwidth, and typically operates from under the crop canopy with degraded network throughput. Moreover, multiple devices streaming simultaneously to the edge creates an \emph{incast}, that additionally overwhelms the above-canopy routers closer to the edge. 
Extracting maximal performance under these conditions requires smart management of the limited network resources. 

We observe that the network management challenges that emerge in farms bear resemblance to datacenters. Like datacenters, farm networks must support a heterogeneous mix of performance critical and background tasks (e.g. remotely controlled robots and sensor data collection). Moreover, unlike typical WiFi settings in homes and enterprises that have unpredictable traffic patterns, farm workloads are more predictable and controlled (in that, they can be explicitly scheduled).\ammar{This should come a lot sooner}
We can therefore draw inspiration from datacenter and WAN traffic engineering (TE) \fixme{add cites} to design a centralized TE engine for \farmernetes. 

A TE system requires reasoning about the available network capacity at each link, and how that gets impacted by different flow allocation (e.g. routing and scheduling) decisions. Doing so is challenging in wireless networks. Unlike wired networks, we cannot reason about network capacity independently for each link. The network capacity (given by the wireless spectrum bandwidth in MHz) is shared by all transmissions to the same receiver (even from multiple different sources), and also by interfering transmissions to other devices that use overlapping channels. Moreover, the amount of network capacity that gets ``used up'' by a (direct or interfering) transmission is not just a function of the transmission rate, but also the distance (transmissions over longer distances at a given datarate consume greater amount of spectrum bandwidth).   

 We introduce the abstraction of ``resource units'' that allows us to systematically reason about these effects. Specifically, it allows us to capture the fraction of wireless network capacity (channel bandwidth) that gets used up at each router by direct and interfering transmissions at varying datarates and distances. 
 %Our abstraction effectively captures the amount of wireless resources needed to transmit at a given rate at varying distances and the amount of resources that are impacted by varying degree of interference. It is uniformly applicable to (and agnostic of) the different underlying wireless mechanisms for spectrum sharing (e.g. TDMA, OFDMA, etc).  
We use this abstraction as the basis of \farmernetes' centralized TE engine to co-optimize three aspects: (i) \emph{Network-aware task scheduling}, where we intelligently schedule networked tasks, determining when they can be started and even pausing or resuming them, based on task deadlines, throughput demands, and the state of the network with respect to device location and other competing (interfering) tasks. (ii) \emph{Network resource allocation}, that includes selecting access points and allocating channels at the 2.4GHz tier, and computing flow routes at the 5GHz tier based on the available network capacity along each route. (iii) \emph{Flow transmission rates}, that are computed based on how the shared wireless spectrum should be divided across contending flows, capturing prioritization and fairness policies (which are non-trivial to realize in a wireless network due to the effects of interference). 


%Our optimization favor access points, channels, and routes that less contended, suffer from less interference from their neighbors, and inflict less interference on neighboring flows. The task scheduling and resource allocation decisions feed into one another and are jointly optimized using a greedy heuristic. \ammar{Discuss}

%\farmernetes incorporates centralized traffic management (TM) to alleviate the above bottlenecks and improve network performance. This is facilitated by the observation that, unlike typical WiFi settings with unpredictable traffic patterns, farm workloads are more controlled and allow room for scheduling. For example, a real-time remote operation for a robot, once requested, need not be scheduled right-away, but can be delayed by a few minutes. \farmernetes' TM uses global knowledge of flow demands and deadlines to co-optimize the start times of flows (even pausing and resuming them again, if allowed), the routes they take, and how the WiFi channels are configured. It takes into account the cumulative effects of transmission distance, congestion, and interference when making these decisions. 
%The TM runs at the edge and communicates with the on-field routers and devices using LoRAWAN. 

%Our TM engine leverages insights from traffic engineering in other domains (e.g. WANs and datacenter \fixme{cites}), but extends them to account for the effects of interference and channel allocation (unique to wireless settings) and temporal scheduling (allowed by the more flexible farm workloads). 
% Similar to classical traffic engineering problem in other domains (e.g. WANs and datacenter), we formulate this as a multi-commodity flow problem, but extend it to account for the effects of interference and channel allocation (unique to wireless settings) and temporal scheduling (allowed by the more flexible farm workloads). We use our formulation to design preliminary strategies to improve the performance of farm networks, and identify interesting future directions in this context \fixme{this needs an update}. \fixme{add something on pre-emption} 

%We build a simulator to simulate the \farmernetes network architecture, and use it to evaluate the significance of different elements (decision knobs) in its traffic management unit. Our simulator draws upon our on-farm measurements to model per-link throughput. It also models the effect of interference and multi-hop performance, that are backed by measurements on real hardware. 

%\textcolor{red}{Deepak: we need a para on how our scheduling improves results. Also, we probably need a name}

%\radhika{We also need to say something about our emulation experiments, perhaps in the list of contributions.}


We build a simulator to simulate the \farmernetes network and to evaluate its traffic manager. We use our on-field measurement traces and control experiments on real hardware (\S\ref{sec:impl}) to guide the models used in our simulator and to validate the correctness of our resource unit abstraction. Our evaluation shows how \farmernetes' TM results in upto 2.5 $\times$ better network utilization and  4 $\times$ better performance for real-time tasks (in terms of throughput normalized by flow demand) when compared with standard wireless mesh strategies. \radhika{update}

While we motivate and evaluate our centralized traffic management engine in the context of farm applications, its design is broadly applicable to other contexts where wireless mesh networks are used to support predictable workloads (e.g. factories, smart cities, mining, etc). 

We summarize our contributions below: 

\noindent $\bullet$ We conduct the first-of-its-kind measurements of WiFi throughput in a cornfield. 

\noindent $\bullet$ Guided by these measurements, we design \farmernetes, a two-tiered network for autonomous farms. 

\noindent $\bullet$ We develop a centralized traffic management engine for \farmernetes, that uses a novel abstraction of resource units to reason about effects of transmission distance and interference that are unique to wireless networks. 

\noindent $\bullet$ We evaluate \farmernetes using trace-driven simulations (informed by experiments on real hardware). 
%Our evaluation highlight the importance of \farmernetes' centralized traffic management decisions. \radhika{revisit}
We will open-source our measurement traces and our simulator. \radhika{update}

%This work does not raise any ethical concerns. 
%\ammar{update as needed}
%\deepak{Should we commit to releasing our measurements and code? People like that.}
% We summarize our contributions below: 

% \noindent $\bullet$ We conduct a survey and literature review to characterize emerging workloads for autonomous farms, identifying the need for a high throughput network that works well even under crop canopy (\S\ref{sec:workload}).

% \noindent $\bullet$ We conduct a first-of-its-kind measurement of WiFi performance in a farm, which highlights the severe impact of crop canopy on network throughput (\S\ref{sec:measurements}).

% \noindent $\bullet$ Guided by our measurements, we design \farmernetes, a unique two-tier network architecture for farms that operates on 2.4GHz under-canopy and 5GHz above canopy (\S\ref{sec:dual-plane}) 

% \noindent $\bullet$ We identify how bottlenecks can quickly emerge on such a network with limited capacity and incast traffic patterns, and design a centralized traffic management engine as part of \farmernetes to improve network performance (\S\ref{sec:te}).  

% \noindent $\bullet$ We build a simulator to simulate the \farmernetes network and to evaluate the significance of different elements (decision knobs) in its traffic management engine. We use our on-field measurements and control experiments on real hardware (\S\ref{sec:impl}) to guide the models used in our simulator. 

%The simulator models per-link throughput based on our on-farm measurements.  We further use control experiments on real hardware to guide our simulator models for interference and multi-hop performance, and to validate the feasibility of implementing some of the proposed techniques (\S\ref{sec:impl}). 

%We do not claim to provide a perfect solution for enabling high throughput network workloads for autonomous farms. We view our work to be a starting point in this exciting domain, with multiple questions open for future research: e.g. do our observed trends extend to other types of crops (beyond cornfields)? how do other connectivity options (e.g. CBRS) perform under canopy, and would our design insights extend to these contexts? how do we deal with variable solar power availability on farms? etc. We discuss these questions further in \S\ref{sec:discussion} \radhika{revisit}.


%\fixme{old text below...}






%Such techniques rely on (a) fine-grained and periodic data collection, e.g. multi-spectral cameras and soil sensors, and (b) individualized actuation by farm robots or drones (e.g. targeted spraying), which often need to be remotely controlled by a human sitting in off-field offices (edge) or via the logic residing in edge servers~\cite{earthsense, cloudrobotics}.





% \begin{itemize}
%     \item Discuss the need for high throughput network:
%     \begin{itemize}
%         \item Motivating examples like teleoperation, fruit harvest, bug spraying etc. 
%         \item Papers from agronomists: some papers included in surveys.
%         \item Discussions/survey with agronomists.
%     \end{itemize}
%     \item Existing networking solutions for farms do not meet these needs
%     \begin{itemize}
%         \item Discuss Farmbeats
%         \item Wifi 6
%     \end{itemize}
%     \item We benchmark performance of Wifi 6 in corn field which shows how Wifi's performance degrades in presence of crops:
%     \begin{itemize}
%         \item 5 GHz is not suitable for under the canopy communication, whereas above canopy range is also only upto 100 meters while giving a decent throughput of 100Mbps.
%         \item 2.4GHz is suitable for under canopy communication but it does not have a lot of bandwidth and has only 3 non-overlapping channels.
%     \end{itemize}
%     \item Our discussions with agronomists and surveys highlight the need for a network capable of providing high throughput real time communication. Further, we also learn that most tasks in such settings have flexibility in deadlines/start times.
%     \item Our measurements and surveys help us envision
% \end{itemize}

%\section{Ethical Concerns}


==> intro-ammar.tex <==
\section{Introduction}

\input{intro-3}

% \begin{enumerate}
%     \item Emphasizing why connectivity in agriculture is a difficult problem
%     \begin{enumerate}
%        \item Need for automation and precision agriculture to improve agriculture practices.
%         \item FCC recognizes connectivity as one of the critical challenges.
%     \end{enumerate}
%     \item Highlight the nature of workloads
%     \begin{enumerate}
%         \item Many edge-drive real-time tasks that require consistently high throughput.
%         \item Many data collection tasks that require the large-scale collection of data over long periods of time i.e. weeks and months.
%         \item Most of the workload is flexible and controllable i.e. possible to even schedule/delay many of the real-time tasks (not always though).
%     \end{enumerate}
%     \item There are layers to network connectivity challenges in agriculture. Farmbeats with TVWS solves the challenge of providing cloud connectivity to the farm. But edge connectivity for devices in the field to edge servers or gateways still exists, especially for such high throughput workloads.
%     \begin{enumerate}
%         \item CBRS and Wi-Fi are two options. One is not necessarily better than the other, in fact, both may be needed in an ideal scenario.
%         \item CBRS may be able to provide consistent, long-range, and high throughput connectivity due to its ability to transmit at higher power. However, it may be constrained by the limited amount of overall bandwidth available (usually a few 10s of MHz).
%         \item Wifi has a much broader band of spectrum available when we count both 2.4 GHz and 5 GHz. Moreover, a small range of Wifi allows for spatial reuse, allowing for much better scalability than CBRS.
%         \item CBRS might be able to provide, single hop, high throughput connectivity but due to its long-range and limited bandwidth, it remains a much more expensive resource reserved for critical tasks such as manual remote recovery. Whereas Wifi should bear the responsibility of all other tasks. 
%     \end{enumerate}
%     \item Just Wifi or a naive Wifi mesh may not be enough.
%     \begin{enumerate}
%         \item Our measurements in the corn field over two seasons show that throughput over a single link can be quite limited, especially for under-canopy communication (a few 10s of Mbps). Throughput degrades further over multi-hop links.
%         \item To support 10s and 100s of devices in an average sized farm, we need careful resource management and we need to solve problems like:
%         \begin{enumerate}
%             \item When to schedule different tasks?
%             \item For any scheduled task, which access point should the under-canopy device connect to? Over which channel? Remember that number of non-overkapping channels can be quite small and selecting same channel for nearby transmissions can cause severe throughput degradation.
%             \item Which path should a flow take to the edge?
%             \item What rate should the flows send at?
%         \end{enumerate}
%         \item On first look, it is tempting to map these problems to various other solved problems like traffic engineering in wired networks.
%         \item However, to begin with, unlike wired networks, "network resources" i.e. the capacity of a link are not fixed and vary depending on the position of the access point and devices, interference from other transmissions. Giving a flow certain throughput has a different effect on other flows depending on the position of devices. Moreover, it not only utilizes resources on the said link but also on links in proximity operating over the same channel. Before, we can manage these resources, we need a way to quantify these effects.
%     \end{enumerate}
%     \item We present a wireless resource abstraction that captures the effect of mobility and interference. We show its effectiveness through real-world experiments.
%     \item Using this abstraction, we design mechanisms to solve the following problems:
%     \begin{enumerate}
%         \item Temporal scheduling of tasks
%         \item Access point assignment and channel selection
%         \item Path selection for scheduled flows
%         \item Rate enforcement
%     \end{enumerate}
% \end{enumerate}



==> intro.tex <==
\section{Introduction}

Emerging precision agriculture and autonomous farming techniques promise to  reduce farm inputs \fixme{perhaps something along lines of reduces wastage} like fertilizers, increase farm yields, and improve agricultural sustainability \cite{king2017future, schimmelpfennig2016farm, the_economist_2016, vasisht2017farmbeats, fcc-report}. For example, bulk spraying of agrochemicals (herbicides, pesticides, etc) can be replaced with targeted chemical application or de-bugging of individual affected plants by robots. In this work, we set out to study the networking requirements of such futuristic autonomous farms, and to what extent they can be met. 

Our study begins with characterizing the network workload for autonomous farms (\S\fixme{XX}). For this, we conducted a survey involving a set of 10 agronomists spanning two institutions, and extensively reviewed relevant literature from agriculture and robotics communities \cite{bogue2020fruit, kamtikar2021fruitarm, tang2020fruitrecognition, sivakumar2021visualnav, insect_detection} \fixme{more here}. The need to periodically collect small amounts of sensor data in farms (e.g. from soil and weather sensors) is well-studied \cite{vasisht2017farmbeats}. In addition, we realized that sensors such as RGB, thermal and hyperspectral cameras might generate 10s to 100s MBs of data per hectare, and that such data might be needed from \emph{under-canopy} sensors (that are placed under the crop canopy) multiple times a day to monitor plant health. More interestingly, workloads for autonomous farms also involve real-time tasks, e.g. autonomously controlled under-canopy robots performing targeted bug spraying, berry-picking, etc. These robots must execute complex planning decisions computed remotely by edge servers (that are typically more powerful than on-field robot devices). The robots must therefore stream rich sensor data at 5-20Mbps from under the canopy to the edge device. 
%Such an edge offload for real-time robot control emerged to be the most popular usecase of farm network in our survey \fixme{?}. 
These workloads emphasize the need for a high throughput network in farms that can support 10s of Mbps of per device even under the crop canopy, as opposed to few tens of Kbps supported by typical farm network options such as LPWAN \fixme{cite}.  


These observations led us to our next question: how much network throughput can we expect to achieve in rural farms? To answer this question, we conducted extensive measurements of WiFi 6 in a cornfield using both 2.4GHz and 5GHz  under different settings (varying distance, varying height of transmission with respect to the crop canopy, etc) and during different times in the farming season. WiFi has been considered as a suitable connectivity medium for rural farms \fixme{cite} due to its ready availability and plug-and-play nature. It was therefore a natural choice for our measurements. %~\footnote{We leave a detailed exploration of other rural connectivity options such as CBRS (which have slightly higher deployment overhead) to future work.}
%Commercial cellular connectivity is limited in rural farms and typical options such as LPWAN are ill-suited for high bandwidth workloads. Use of private spectrum such as CBRS and TVWS, had a greater setup cost which precluded us from using them. WiFi has more of a plug-and-play property making it an easier choice for our measurements (and potentially also for real-world deployments in farms). Nonetheless, it will be interesting to see how our insights extend to CBRS (left for future work). \fixme{need to fix and discuss.}}  
Unlike typical settings where WiFi is used, farms do not suffer from interference from external sources, thereby allowing use of all the WiFi channels \fixme{fix this line}. However, the network throughput and range can be impacted by the presence of crop canopy. Ours is the first measurement study to characterize this impact of crop canopy on network throughput.

We find that 5GHz WiFi is unable to work well under-canopy, with the effective throughput degrading to zero beyond a short distance of 40m. In contrast, 2.4GHz WiFi is more robust, sustaining upto \fixme{15 Mbps} of average throughput at a distance of \fixme{80 meters}. We further observed that small spatial variations in device location under the crop canopy can impact network throughput. While one would expect 2.4GHz to be more robust to obstacles, we were surprised by the severity with which the performance of 5GHz (configured to make use of the 160 MHz wide band through channel bonding) degrades under-canopy. For transmissions above the crop canopy, on the other hand, 5GHz fared significantly better than 2.4GHz due to its use of wider channels (and more bandwidth), achieving upto 100 Mbps of throughput at distance of 100 m (2.5 $\times$ higher than 2.4GHz). However, this was still 2 $\times$ lower than the throughput 5GHz could have achieved in the absence of crop canopy! While the timing of the farming season impacted the network throughput (due to difference in moisture content in the crops), the high-level trends were consistent. 

The insights from these measurements indicate a unique network design for autonomous farms: a multi-hop mesh of routers placed above canopy (e.g. on poles) that operate on two planes: (i) the 2.4GHz plane, where they talk to the under-canopy devices (e.g. robots) over 2.4GHz channels, and (ii) the 5GHz plane, where the traffic is routed at 5GHz above the canopy across the mesh. So an autonomously operated under-canopy robot or sensor would stream its sensed data over a 2.4GHz channel to one of the routers in its range. The data will then be routed across the mesh of above-canopy routers using 5GHz to the edge servers in near vicinity (farmer's home or some service's parked trucks). 

We next note that capacity is fundamentally limited in such a network -- the presence crop canopy degrades throughput on both the 2.4GHz plane under-canopy and the 5GHz plane above canopy. In particular, we observe that even a handful \fixme{3-4?} of co-located under-canopy devices can overwhelm the 2.4GHz link to a router. Over-provisioning the network by adding more routers cannot help in this case as 2.4.GHz is restricted to using three non-overlapping channels, and neighboring routers operating on the same channel would interfere with one another. Likewise, bottlenecks can quickly emerge in the 5GHz plane due to incast pattern of the workload when multiple on-field devices wish to stream data to the edge servers. Vanilla strategies \fixme{better word} like scheduling flows as and when they are requested and shortest-path routing are insufficient to meet the demands of farm workloads, even at a small scale with a handful of devices (with the problem exacerbating with increasing scale of autonomous operations). 


Here we observe that, unlike typical WiFi settings with unpredictable traffic patterns, farm workloads are more controlled and allow room for scheduling (e.g. a real-time remote operation for a robot, once requested, need not be scheduled right-away, but should proceed with minimal interruptions once it has been scheduled.). We can therefore improve the effective network utilization (and throughput) through careful traffic engineering and flow scheduling, driven by flow demands and deadlines. This includes tuning the start times of flows, the routes they take, and the channel allocations in both the 2.4GHz and 5GHz planes. Similar to classical traffic engineering problem in other domains (e.g. WANs and datacenter), we formulate this as a multi-commodity flow problem, but extend it to account for the effects of interference and channel allocation (unique to wireless settings) and temporal scheduling (allowed by the more flexible farm workloads). We use our formulation to design preliminary strategies to improve the performance of farm networks, and identify interesting future directions in this context. \fixme{add something on pre-emption} \fixme{revisit}

We summarize our contributions below: 

\noindent $\bullet$ We characterize emerging workloads for autonomous farms, thereby identifying the need for a high throughput network that works well even under crop canopy.

\noindent $\bullet$ We conduct a first-of-its-kind measurement of WiFi performance in farms, which highlights the severe impact of crop canopy on network throughput.

\noindent $\bullet$ Guided by our measurement results, we propose a unique network design for autonomous farms that operates on 2.4GHz under-canopy and 5GHz above canopy. 

\noindent $\bullet$ We identify how bottlenecks can quickly emerge on such a network with limited capacity, and design flow scheduling and traffic engineering techniques to improve network performance. 

We do not claim to provide a perfect solution for enabling high throughput network workloads for autonomous farms. We view our work to be a starting point in this exciting domain, with multiple questions open for future research: e.g. do our observed trends extend to other types of crops (beyond cornfields)? how do other connectivity options (e.g. CBRS) perform under canopy, and would our network design extend to these contexts \fixme{discuss}? how do we deal with variable solar power availability on farms, and extend our scheduler to deal with device mobility? etc. 


\fixme{old text below...}






%Such techniques rely on (a) fine-grained and periodic data collection, e.g. multi-spectral cameras and soil sensors, and (b) individualized actuation by farm robots or drones (e.g. targeted spraying), which often need to be remotely controlled by a human sitting in off-field offices (edge) or via the logic residing in edge servers~\cite{earthsense, cloudrobotics}.





\begin{itemize}
    \item Discuss the need for high throughput network:
    \begin{itemize}
        \item Motivating examples like teleoperation, fruit harvest, bug spraying etc. 
        \item Papers from agronomists: some papers included in surveys.
        \item Discussions/survey with agronomists.
    \end{itemize}
    \item Existing networking solutions for farms do not meet these needs
    \begin{itemize}
        \item Discuss Farmbeats
        \item Wifi 6
    \end{itemize}
    \item We benchmark performance of Wifi 6 in corn field which shows how Wifi's performance degrades in presence of crops:
    \begin{itemize}
        \item 5 GHz is not suitable for under the canopy communication, whereas above canopy range is also only upto 100 meters while giving a decent throughput of 100Mbps.
        \item 2.4GHz is suitable for under canopy communication but it does not have a lot of bandwidth and has only 3 non-overlapping channels.
    \end{itemize}
    \item Our discussions with agronomists and surveys highlight the need for a network capable of providing high throughput real time communication. Further, we also learn that most tasks in such settings have flexibility in deadlines/start times.
    \item Our measurements and surveys help us envision
\end{itemize}

==> problem.tex <==
% \subsection{Problem Statement}

% Measurements from the \S \ref{sec:measurements} hint towards a mesh network since the range of a single AP is too short. Such a network must also utilize the 2.4GHz band for the first hop between under-the-canopy devices and nearby AP, and use the 5GHz band for AP-AP links. Despite all this, bottlenecks can emerge quite easily e.g. 100 Mbps over 160 MHz wide 5GHz band may only sustain a handful of real-time flows, especially in the typical scenario of in-cast to edge. Similarly, without careful channel allocation for 2.4GHz interfaces of routers, the first hop can itself be a bottleneck. The flexible nature of the workload allows us to apply different resource management techniques. We imagine a scheduler that temporally schedules tasks based on their priorities and deadlines, finds network path keeping into account interference, and allocates channels.


\section{Problem Formulation}
\label{appendix:problem_formulation}
In this section, we formulate the problem of scheduling tasks, finding optimal routes for them, and doing optimal channel allocation. This can be formulated similar to the multicommodity flow problem. Consider the mesh network to be a graph $G = (V, E)$ where $v \in V$ is a router and $e(u,v,b) \in E$ is an edge between $u \in U$ and $v \in V$ and $b$ is for the interface since $u$ and $v$ may connect over 2.4 GHz or 5 GHz interfaces. For each vertex $v \in V$, each interface $b$ has an upper limit on bandwidth $c(v,b)$. Consider $K$ to be a set of tasks, where $k_i \in K$ can be defined as $k_i(s_i, t_i, d_i, st_i, dd_i, dr_i)$ where $s_i$ and $t_i$ are source and destination for the flow respectively, $d_i$ is its demand, and $st_i$, $dd_i$ and $dr_i$ are start time, deadline and duration of the task \footnote{In this formulation we consider only real-time flows for simplicity.}. To add dimension of time, consider $t \in T$ to be a time interval (e.g. 1 minute) and $T$ be the ordered set of all contiguous time intervals. Let $f_i(u,v,b,t)$ be a boolean variable denoting whether flow $k_i$ uses the edge $e(u,v,b)$ in its path during time interval $t$. Let $\theta_i(t)$ be another boolean variable suggesting whether $k_i$ flow is scheduled at time interval $t$. Finally, let $h(u,b,t)$ be a variable denoting channel used by $u \in V$ node for $b$ interface at time interval $t$, and its value is picked from fixed sets $h(u, 2.4, t) \in Channels_{2.4}$ and $h(u, 5, t) \in Channels_{5}$.

The following objective function maximizes the effective throughput of our network.

\begin{equation}
    \max_{f_i, \theta_i, h} \sum_{t \in T} \sum_{k_i \in K} f_i(u,v,b,t) \theta_i(t) d_i
\end{equation}

The first few constraints are to respect the bandwidth capacities. The incoming and outgoing traffic on a node $v \in V$ must not exceed its interference deducted capacity $c'(v,b,t)$ at time $t$:

\begin{equation}
    \begin{alignat}{2}
    \forall t \in T \forall (u,v,b) \in E: \sum_{k_i \in K} f_i(u, v, b, t) d_i \theta_i(t) \\
    \leq c'(u,b,t), st_i \leq t \leq dd_i
    \end{alignat}
\end{equation}
\begin{equation}
    \begin{alignat}{2}
    \forall t \in T \forall (u,v,b) \in E: \sum_{k_i \in K} f_i(u, v, b, t) d_i \theta_i(t) \\
    \leq c'(v,b,t), st_i \leq t \leq dd_i
    \end{alignat}
\end{equation}
    
\begin{equation}
    \begin{alignat}{2}
        \forall v \in V: c'(v,b,t) = c(v,b) - \sum_{u in V} Interference (u, v),\\
        h(v,b,t) = h(u,b,t)
    \end{alignat}
\end{equation}

Following constraints ensure flow conservation at transit nodes, source nodes and destination nodes respectively:

\begin{equation}
    \begin{alignat}{2}
        \forall t \in T \forall k_i \in K: \sum_{u \in V}f_i(u,v,b,t) \theta_i(t) - \\
        \sum_{u \in V}f_i(v,u,b,t) \theta_i(t) = 0, u \neq s_i, t_i
    \end{alignat}
\end{equation}

\begin{equation}
    \begin{alignat}{2}
        \forall t \in T \forall k_i \in K: \sum_{u \in V}f_i(s_i,u,b,t) \theta_i(t) - \\
        \sum_{u \in V}f_i(u,s_i,b,t) \theta_i(t) = 1
    \end{alignat}
\end{equation}

\begin{equation}
    \begin{alignat}{2}
        \forall t \in T \forall k_i \in K: \sum_{u \in V}f_i(t_i,u,b,t) \theta_i(t) - \\
        \sum_{u \in V}f_i(u,t_i,b,t) \theta_i(t) = -1
    \end{alignat}
\end{equation}

Total amount of time a flow is scheduled should be no more than the duration of the task:

\begin{equation}
    \forall k_i \in K: \sum_{t \in T} \theta_i(t) \leq dr_i
\end{equation}

Lastly, we have constraints on our variables:

\begin{equation}
    f_i(u,v,b,t) \in \{0,1\}
\end{equation}

\begin{equation}
    \theta_i(t) \in \{0,1\}
\end{equation}

\begin{equation}
    h(u,2.4,t) \in Channels_{2.4}
\end{equation}

\begin{equation}
    h(u,5,t) \in Channels_5
\end{equation}

The flow commodity problem when $f_i$'s value is discrete is a well-known NP-hard problem. Additionally, the channel allocation aspect of the problem is also NP-hard since it is essentially a graph coloring problem.


\section{Throughput and Interference Modeling}
\label{appendix:modeling}

Our simulator needs to model throughput any transmission would get at different distances. We fit logarithmic curves on our dataset from figure \ref{fig:distance1} to make models for different modes e.g. 2.4 GHz under the canopy. Throughput is modeled in simulation using these curves. $Throughput(distance, mode)$ gives throughput over all the resources available for the respective mode. From this we can calculate the amount of resources needed to support a particular flow of demand $x$ Mbps from device $r_s$ to $r_d$ over mode $m$, which is given as:
\begin{equation*}
    \begin{alignat}{2}
        $ResourceUnits(x, r_s, r_d) = \frac{x}{ Throughput(Distance(r_s, r_d), m)}$
    \end{alignat}
\end{equation*}

Then the interference from the transmission of $x$ Mbps between router $r_s$ and $r_d$ has an effect on resources available to $r_n \in Neighbours(r)$ as follows: If $r_n$ is closer or at same distance from $r_s$ as $r_d$ is from $r_s$, then the affect of $Interference(x, r_s, r_d, r_n) = ResourceUnits(x, r_s, r_d)$. However, if $r_n$ is further away then the affect of interference slowly degrades. We model this degradation based on our throughput models as well. We assume that interference degrades at the same proportion as the throughput does w.r.t distance. We divide the amount of resources needed for transmission between $r_s$ and $r_d$ by the amount of resources needed if transmission of $x$ Mbps was from $r_s$ to $r_n$ instead. This gives us proportional degradation in throughput due to increase in distance, this is multiplied with the actual amount of resources used by $r_s$ to send $x$ Mbps to $r_d$.

\begin{equation*}
    \begin{alignat}{2}
        $Interference(x, r_s, r_d, r_n) = \frac{ResourceUnits(x, r_s, r_d)}{ResourceUnits(x, r_s, r_n)} &\\ \times  ResourceUnits(x, r_s, r_d)$
    \end{alignat}
\end{equation*}

Lastly, contention on a router $r$ is given by the amount of resources needed by router $r$ to support all flows passing through it and the effect of interference from the neighboring nodes.

\begin{equation*}
    \begin{alignat}{2}
        $Contention(r) = \sum_{f \in Flows_r} ResourceUnits(f, r, \_) + &\\ \sum_{r_n \in Neighbours} \sum_{f \in Flows_r_n} Interference(f, r_n, \_, r)$
    \end{alignat}
\end{equation*}

\begin{figure*}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat[Overall Throughput]{\includegraphics[width=0.34\textwidth]{figures/local-data.pdf} \label{fig:local_data}}
\subfloat[Per-flow Throughput]{\includegraphics[width=0.34\textwidth]{figures/local-qos.pdf} \label{fig:local_qos}}
\vspace{-10pt}
\caption{Farmernetes' improvements in overall and per-flow throughput over baseline for a localized workload.}
\vspace{-10pt}
\label{fig:local}
\end{figure*}



==> resource-unit-old.tex <==
Throughput for Wifi: The maximum throughput over a Wifi connection can be calculated by Shannon's law as~\footnote{While actual formula is $\log_2(1 + \frac{S}{N})$, we can ignore 1 if $\frac{S}{R} > 1$.}:

$$Throughput = BW \times \log_2 (\frac{S}{N}) = BW (\log_2(S) - \log_2(N))$$ 

Where S is the signal strength between sender and the receiver, and N is base noise and interference from other transmission. BW is the bandwidth of the channel in Hz. While this is the maximum throughput a link can sustain, any throughput smaller than this will utilize a proportional fraction of the bandwidth since it will try to access the medium only that often.

\begin{figure}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat[Normalized throughput of two senders add up to 1]{\includegraphics[width=0.23\textwidth]{figures/distance-throughput-abstraction.pdf} \label{fig:distance-throughput}}
\subfloat[We can divide resources in any fraction between flows (1:1 here)]{\includegraphics[width=0.23\textwidth]{figures/distance-throughput-abstraction-fair.pdf} \label{fig:distance-throughput-fair}}
\vspace{-10pt}
\caption{Micro benchmark to verify eq. \ref{eqn:throughput-distance}}
\vspace{-10pt}
\label{fig:distance-abstraction}
\end{figure}

\begin{itemize}
    \item Definition of resource unit: A transmission of X Mbps between devices A and B consumes a certain amount of wireless bandwidth not only at A and B but also at neighboring devices due to interference. 1 resource unit is the normalized bandwidth of a device. This way, each device initially has 1 resource unit each and each transmission between any pair of nodes consumes fractional amount of resource units at multiple devices. Let us take a guiding example of a sender S transmitting X Mbps to a receiver R placed distance d away.
    \item \textbf{Resource Units Consumed at S and R: } The amount of resource units consumed at sender S or receiver R is a function of the distance between them. If the distance is higher more resource units (or bandwidth) will be consumed to sustain the same data rate. We know how throughput degrades with distance for different bands and settings, so we can calculate the amount of bandwidth consumed to send X Mbps between S and R as:
    \begin{equation}\label{eqn:throughput-distance}
    r_{S \longrightarrow R} (X, d) = \frac{X}{Throughput_{S \longrightarrow R}(d)}\tag{1}
    \end{equation}

    For 802.11 ac, this fraction represents the fraction of time when this flow would get access to the channel using CSMA. So this fraction is the same for both sender and receiver. Our real-world experiments verify that this abstraction holds. We placed a router above the canopy and two senders 10 meters away from the router, under the canopy, and measured throughput separately and then together. We moved one sender 20 meters away and repeated this and so on. Figure \ref{fig:distance-throughput} shows the throughput from each sender normalized by the total throughput they got separately at each distance, this adds up to 1 as predicted by the abstraction. It is interesting to note how the sender that is further away gets lower and lower share of bandwidth. In another run of the experiment, we hand pick the rate for both senders based on their independent throughputs to ensure each of them get half of resource units. Figure \ref{fig:distance-throughput-fair} shows that flows share bandwidth fairly now.

\begin{figure}
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}
\centering
\subfloat[Stationary sender's throughput]{\includegraphics[width=0.23\textwidth]{figures/primary_throughput_prediction.pdf} \label{fig:distance-throughput}}
\subfloat[Moving sender's throughput]{\includegraphics[width=0.23\textwidth]{figures/secondary_throughput_prediction.pdf} \label{fig:distance-throughput-fair}}
\vspace{-10pt}
\caption{Actual throughput versus throughput predicted by eq. \ref{eqn:interference} after accounting for interference from other flow.}
\vspace{-10pt}
\label{fig:interference-abstraction}
\end{figure}

  
    \item \textbf{Resource Units Consumed at Neighbour I: }This transmission also has an impact on neighboring nodes (say I) in the form of interference. If we assume maximum signal power and minimum noise level is the same across the farm. From Shannon's law, we know throughput is linearly proportional to the log of signal strength. As the distance between sender and receiver increases, the $log_2(S)$ decreases proportionally to the throughput decrease. Similarly, as the $log_2(N)$ increases due to interference, it results in a proportional reduction in throughput as well. Interference from another transmission from I to R can then be calculated using the throughput-distance curve. The interfering signal should have degraded by the same ratio as throughput from I to R would have degraded over distance d'. Thus resource units consumed due to interfering signal can be calculated as:

    \begin{equation}\label{eqn:interference}
    \delta_{I \longrightarrow R} = \frac{Throughput_{I \longrightarrow R (d')}}{MaxThroughput}\tag{2}
    \end{equation}
    
    % $$\delta_{I \longrightarrow R} = \frac{Throughput_{I \longrightarrow R (d')}}{MaxThroughput}$$

    Here $MaxThroughput$ is the maximum throughput. If I is sending only a fraction of time i.e. $r_I$, then we can scale $\delta_{I \longrightarrow R}$ down by $r_I$. We use these equations to predict the throughput of two flows in the presence of interference from each other through real-world experiments. We have two routers operating independently on the same channel placed above the canopy 50 meters apart. We have two senders placed under the canopy 10 meters away from the first router. We move one sender 10 meters away from the first router and toward the second router, while the other sender stays at the same place. We measure throughput between each device pair separately as baselines and then measure throughput while the stationary sender sends to the first router at maximum rate and the moving router sends at maximum rate to the second router. Given the throughput of one flow, we use above equations to predict the throughput for the other flow. Figure \ref{fig:interference_abstraction} shows how well we are able to predict the effect of interference on a device.
    % Where $MaxThroughput$ is the maximum achievable throughput i.e. throughput at the highest signal strength. If the interfering signal consumed $r_{I}$ resource units at $I$ to transmit, then by the time this signal reaches R, it would consume the following amount of resources at R:
    % $$r_{R(I)} = r_{I} \times \delta_{I \longrightarrow R} = r_{I} \times \frac{Throughput_{I \longrightarrow R (d')}}{MaxThroughput}$$
    \item \textbf{Multiple Source of Interference: } Any single source of interference consumes resource unit given by the equation. However, what happens when we have multiple sources of interference? Let's say we have $n$ sources of interference, with resource units for each consumed given by:
    $$\delta_{i} = \frac{Throughput_{i(d')}}{MaxThroughput}$$
    % $$r_{R(i)} = r_i \times \delta_i$$

    By using Shannon's equation from earlier and ignoring base noise, we can define $\delta_i$:

    $$\delta_i = \frac{log_2(I_{i \longrightarrow R})}{C}$$

    where $I_{i \longrightarrow R}$ is the power of interfering signal from device $i$ to R and $C$ is a constant for the log of minimum power needed for maximum throughput which can be easily found. Re-arranging this for $I_{i \longrightarrow R}$, we get:
    $$I_{i \longrightarrow R} = 2^{\delta_i \times C}$$

    % If each interfering sender transmits a fraction of time depending on how much data it is sending i.e. how many of its resource units, it is using, given by $r_i$. Then power of its interfering signal can be called by $r_i$ to get final power of this signal:
    % $$I_i = r_i \times I_{i \longrightarrow R} = r_i \times 2^{\delta_i \times C}$$
 
    The expected power of cumulative interfering signals is simply the sum of all signals, so we have:

    $$I = \sum_i  2^{\delta_i \times C}$$

    For R, the resource units utilized at R by all these interfering transmissions is given by:
    $$\delta_R = \frac{\log_2(\sum_i 2^{\delta_i C})}{C}$$

    To simplify this calculation, we overestimate interference slightly by replacing $\log_2(\sum_i 2^{\delta_i C}) \leq \log_2(\sum_i 2^{\delta_i})^C$:

    $$\delta_R = \frac{C \log_2(\sum_i 2^{\delta_i})}{C} = \log_2(\sum_i 2^{\delta_i})$$

    $\delta_i$ here is resources used by an interfering sender sending at full-rate. If sender only sends at fractional rate $r_i$, we can scale down resources used to $\delta_i \times r_i$.
    % \ammar{C cannot come out now even if we use the inequality we discussed previously because $r_i$ is different for each $i$ (although between 0 and 1). Moreover, this equality does not do very well for the measurements I have. Instead following holds better:
    % $$r_R = \frac{\log_2(\sum_i 2^{\delta_i r_i C})}{C} \geq \log_2(\sum_i 2^{\delta_i r_i})$$
    % This can only work if we have $r_i \times \delta_i = \frac{\log_2(I_i)}{C}$ but I am not sure how that works}
\end{itemize}


==> twotier-old.tex <==
\section{\farmernetes' Two-Tiered Architecture}
\label{sec:two-tier}

% \radhika{todo: replace plane with tier whereever we find it}
% \begin{figure*}
% \centering
% \captionsetup{justification=centering}
% \captionsetup[subfigure]{justification=centering}
% \centering
% \subfloat{\includegraphics[width=0.44\textwidth]{figures/farmnet1.pdf} \label{fig:dualplane5ghz}}
% \subfloat{\includegraphics[width=0.44\textwidth]{figures/farmnet2.pdf} \label{fig:dualplane2ghz}}
% \vspace{-10pt}
% \caption{Dual Plane Network with 2.4 GHz plane for first hop connectivity for under the canopy robots and 5 GHz plane for routing traffic to edge. \textbf{(a)} Traffic engineering is needed in 5 GHz plane \textbf{(b)} 2.4 GHz plane requires careful AP selection and channel allocation. \ammar{need to be fixed}}
% \vspace{-10pt}
% \label{fig:dualplane}
% \end{figure*}



\farmernetes design is guided by our observations from \S\ref{sec:measurements}, which indicate a clear division of responsibility between the 2.4Hz and the 5Ghz bands. \farmernetes architecture therefore comprises of a multi-hop mesh of WiFi routers placed above the crop canopy (e.g. mounted on poles) in a grid topology (as shown in Figure \ref{fig:dualplane}). These routers operate in two distinct tiers : \emph{(1) 2.4GHz under-canopy:} where the
%\paragraphb{(1) 2.4GHz under-canopy data plane:}
\farmernetes routers communicate with under-canopy robots and sensors over the 2.4GHz interface, and
%One could argue that the need for under-canopy communication can be eliminated by mounting the WiFi antennas over the canopy height for each robot. However, this is not a practical alternative, as doing so can damage crops and hinder the under-canopy robot's motion and ability to perform tasks.\radhika{maybe cut this point if mentioned in the intro}   
\emph{(2) 5GHz above-canopy:} where the \farmernetes routers use the 5GHz interface to route traffic across the mesh above the crop canopy in order to communicate with the edge servers (or with other on-field devices).
%One could again argue that the above canopy routers can be connected using Ethernet cables -- this is again not practical in a farm setting as the cables may interfere with growing crops. Moreover, this would hinder the agility of the network infrastructure (the need for which is discussed below).  \radhika{makes sense? better reason?} 
%\paragraphb{(2) 5GHz above-canopy data plane} 

This two-tier architecture can be supported using commodity WiFi routers that are typically dual-band, having one interface each for 2.4GHz and 5GHz. The 2.4 GHz interface operates in Infrastructure mode and acts as Access Point (AP) for robots whereas the 5 GHz interface operates in ad-hoc mode to form a mesh.
% \radhika{Ammar, please add a line here on how you are configuring the routers (AP mode for 2.4GHz and adhoc mode (?) for 5GHz} \radhika{can commodity WiFi routers support LoRA? } \ammar{no, we need to add attachments as in \S 6.3}

\paragraphbq{Why the two tiers?} 5GHz does not work under-canopy, restricting under-canopy transmissions to 2.4GHz. However, a question that remains is whether 2.4GHz could have been used above canopy to augment 5GHz throughput? Doing so might also allow two neighboring 5GHz routers to operate on different channels (to minimize interference) with the 2.4GHz interface acting as a bridge for sending flows between them. We considered adopting this idea, but dismissed it when our evaluations revealed that the longer range of 2.4GHz above canopy makes it ill-suited for routing in the mesh, and severely impacts the under-canopy transmissions (that invariably interfere with the long range above canopy 2.4GHz transmissions that must use one of the three non over-lapping channels). This reinforces \farmernetes' strictly tiered architecture.  
\radhika{corollary question: 5GHz under canopy for short range -- also bad, we have results...}

%\radhika{rewrite and sharpen the discussion below, perhaps covering separate set of challenges for 2.4 and 5GHz, each of which require separate solutions}  
%\paragraphb{(3) LoRAWAN-based Management Plane} 


% \paragraphb{Deployment Models} There can be two deployment models for such a network:

% \paragraphi{(i) Farmer-owned.} In this model, the farmer owns and deploys the network infrastructure and the smart agricultural devices. Many farms are savvy enough to potentially support such a model \radhika{reword this sentence and cite that farmer's website, and the sugar plantation thing}.

% \paragraphi{(ii) Service-based.} We envision a more common deployment model would be the one where the farmers do not buy and deploy the network and the smart agriculture infrastructure themselves. This is instead taken care of by an external service that brings in all the networking equipment along with robots and other devices (such digital farming services already exist today and are becoming increasingly popular \radhika{find cite}). Such a service may host edge servers either in trucks parked near the farm or a building with a power supply near the farm, and can deploy the network and the smart devices in specific areas of the farm that they are servicing on a given day. 



%\paragraphb{Design Considerations and Challenges} \radhika{maybe need a better paragraph heading} Deploying such a network requires tackling the following key design considerations and challenges. 

% 



%\paragraphi{Coverage.} Another design consideration is the level of coverage that the network infrastructure must provide. Some farmer-owned deployments may choose to install the network so as to have complete coverage over the entire farm, such that devices across the field are able to simultaneously operate . Assuming each router is placed \fixme{XXm} apart, providing coverage for an \fixme{XX} acre field would require \fixme{XX} routers. This would cost \fixme{\$XX}, which is relatively inexpensive, given that a single autonomous robot costs  \fixme{\$YY}. Another alternative is to provide coverage over a smaller region of the farm, moving the infrastructure to service different parts of the farm on different days (such a model can be adopted not just in service-based deployments but also in farmer-owned deployments). 

%\paragraphi{Router Density.} 

\radhika{mention how many routers needed to cover an average farm}
\radhika{deduplicate challenges below from what we have written earlier.}
Our measurements in \S\ref{sec:measurements} show that the throughput degrades with increasing distance of transmission. This seemingly indicates that increasing the density of routers can increase the effective network throughput (although, also the deployment cost). However, increasing the router density beyond a certain point is detrimental as it increases interference between routers sharing the same spectrum on overlapping channels. In other words, capacity is fundamentally limited by spectrum in a wireless mesh network, and over-provisioning cannot help. This challenge manifests in different forms in the 2.4GHz and 5GHz tier, requiring different traffic management solutions. 


\paragraphb{Challenges in 2.4GHz tier}  
%While 5GHz fails to wok under-canopy beyond a short distance of 40m, 2.4GHz has limited under-canopy bandwidth (\fixme{XX}Mbps at 40meters, and progressively lower at increasing distances). 
A given router, serving multiple co-located under-canopy devices can only operate over a single channel at which its 2.4GHz interface is configured. So devices transmitting to the same router must share the spectrum over the same channel. Their effective throughput depends on their relative distance to the router. 
Load-balancing devices across multiple neighboring routers (and not necessarily picking the nearest router as the access point) can alleviate some of the contention. However, 2.4GHz has only three non-overlapping channels (channel 1,6, and 11). So while neighboring routers can be configured with different channels to minimize interference, with a choice of only three non-overlapping channels, contention cannot be eliminated when there are four or more active devices in each-other's range, even when they are transmitting to different routers. The choice between picking a nearer router operating on a more contended channel, and a more distant router operating on a less contended channel, must further account for the relative impact of contention and distance on effective throughput. 

%This might increase the transmission distance (and therefore the effective throughput).... More importantly, 2.4GHz has only three non-overlapping channels. So while neighboring routers can be configured with different channels to minimize interference, with a choice of only three non-overlapping channels, interference cannot be eliminated when there are four or more active devices in each-other's range.  

Similar issues materialize in wireless meshes in other settings (e.g. when picking access points and configuring channels in homes or enterprises \cite{rozner2007traffic}). However, these issues are more acute for under-canopy transmissions in a farm, where 5GHz does not even work, and 2.4GHz throughput is very limited to begin with. Nonetheless, unlike typical WiFi meshes in homes and enterprises, \farmernetes can alleviate these issues by leveraging the more controlled farm workloads to stagger flows and to configure the choice of access points and channel allocations in a centralized manner (as detailed in later in this \S\ref{sec:heuristics})

%\farmernetes's centralized traffic manager (\S\ref{sec:scheduling}) tunes three key knobs so as to  maximize the effective throughput in the 2.4GHz tier: (i) the time of scheduling a flow, (ii) which router to pick as the access point, and (iii) how to allocate channels across the routers. 

\paragraphb{Challenges in 5GHz tier}  
The 5GHz interface, used for transmissions above canopy, must operate over the same channel at each router. In particular, a flow transmitted using channel $C$ by one router can be received by the next hop only on the same channel $C$. So all hops for a given flow must be configured to use the same channel. Moreover, all flows passing through the same router must use the same channel, as a given 5GHz interface at a router can only be configured to use a single channel. The combination of these two factors quickly cascade into operating the entire network on the same 5GHz channel.
\farmernetes uses channel bonding to maximize the bandwidth for that channel. However, bottlenecks easily emerge in the 5GHz tier,  when multiple devices simultaneously stream data to the edge server, creating an incast and overwhelming the routers closest to the edge. The interference caused by neighboring routers (all operating on the same channel) further aggravates the issue. As per our measurements, the throughput for above canopy 5GHz transmissions is limited to 100Mbps at 80m to begin with. Combining the effects of interference, fewer than 10 devices simultaneously transmitting to the edge at 10Mbps would end up overwhelming the network capacity.~\footnote{Using tri-band routers that support two 5GHz interfaces enables using an additional channel in the 5GHz tier, thereby doubling the available bandwidth. Nonetheless, the issue of limited capacity, that is aggravated by incast, still holds, especially as the scale of deploying smart agricultural devices increases.}

\farmernetes deals with this challenge by again leveraging global knowledge of farm workloads to stagger flows when possible, and to compute flow routes in a centralized way by taking into account the effects of contention and interference. Our evaluation in \S\ref{sec:eval} shows how the routes computed by \farmernetes lead to better throughput than computing routes based on shortest hop count~\cite{chakeres2004aodv, johnson2001dsr, dsdv, olsr} or better link qualities~\cite{etx-roofnet, aguayo2004roofnet} (the standard policies for decentralized routing in WiFi meshes).      

\radhika{for the above, shrink the part about challenges, and highlight the resource allocation decision at each tier.}


%Must use same channel. Link between two routers shared by multiple flows, and they would cause interference on neighboring routers. Bandwidth reduces with increasing range and causes interference. All of these effects must be taken into account when configuring routes. \farmernetes leverages global knowledge of flow requirements to centrally compute routes by accounting for these factors. Also mention incast.... 
%can't use 2.4GHz for bridging...

%So the placement of routers must balance the trade-off between transmission range, effects of interference and deployment costs. 

%The effective throughput at a given range (and the ensuing impact of interference) may vary across the growing season -- the agility of network infrastructure can be leveraged to adjust the distance between routers. \radhika{can we give some numbers here? e.g. why we feel 80-100m is a good distance?}

%\paragraphi{Spectrum-limited Capacity.} \radhika{split into two paragraphs: challenges in 2.4GHz tier and 5GHz tier} As pointed above, capacity is fundamentally limited by spectrum in such a wireless network. This holds for both the 2.4GHz plane (that has only three non-overlapping frequency channels) and for the 5GHz plane (that must operate on the same channel to form a mesh). As a result bottlenecks can emerge in the 2.4GHz plane when as few as four co-located devices simultaneously transmit data using the same or neighbouring routers. Likewise, bottlenecks can emerge in the 5GHz plane when multiple devices simultaneously stream data to the edge server, creating an incast. \farmernetes' traffic management engine \radhika{management plane} (discussed in more details in the next section) is designed to alleviate such bottlenecks via careful flow scheduling, route selection on the 5GHz plane, and channel allocation on the 2.4GHz plane.  

% \paragraphi{Capacity Limitation in the 2.4GHz Plane.} The key reason for limited spectrum capacity in the 2.4GHz plane stems from the fact that the 2.4GHz band has only three non over-lapping channel. So as few as four co-located devices (using either the same or neighbouring routers) would start competing for network capacity, which is limited to begin with for under-canopy transmissions. Careful spectrum management, channel allocation, and flow scheduling are needed to utilize the 2.4 GHz plane properly. 

% \paragraphi{Capacity Limitation in the 5GHz Plane in the 5GHz plane} All routers must operate on the same frequency channel in the 5GHz plane to form a mesh. Incast traffic patterns and interference can result in the 5 GHz plane becoming the bottleneck.



%A typical router usually has one interface each for the 2.4 GHz and the 5 GHz bands. Given the limited amount of bandwidth and independent channels in the 2.4 GHz band, its interface should be reserved for communication with under-the-canopy robots i.e. the first hop. This leaves the 5 GHz interface to communicate with other routers placed above the canopy. Thus our network operates in two different planes. Both planes have different jobs and different challenges. In the 2.4 GHz plane, the challenge arises because of the small number of non-overlapping channels. The first hop can easily become a bottleneck in the presence of other 2.4 GHz flows on the same router or neighboring routers. Careful spectrum management and channel allocation are needed to utilize the 2.4 GHz plane properly. In the 5 GHz plane, all routers operate on the same frequency channel to form a mesh. Incast traffic patterns and interference can result in the 5 GHz plane becoming the bottleneck. Therefore, traffic engineering and resource management techniques are required for this plane.

%Design considerations: 

% \paragraphb{Placement of routers} Router placement needs to take into account workload and Wifi characteristics like interference. Throwing more routers into the mix does not scale the throughput as routers eventually need to share the same spectrum. Similarly, placing routers closer to each other may actually be detrimental to the throughput due to increased interference across hops for the same flow (as shown in \S \ref{sec:impl}). Thus to achieve some feasible target end-to-end throughput, routers need to
% placed carefully taking into account factors like surroundings and interference.

% \paragraphb{Coverage} 


% \paragraphb{Agility}  

% \paragraphb{Network Management} As discussed bottlenecks can emerge in both planes for our dual-plane network, so we must do careful resource allocation. Given the flexibility in nature of most autonomous farm jobs w.r.t. start times and deadlines, most flows can allow for temporal scheduling. This scheduling can improve overall network resource utilization greatly by efficiently dividing workload across time. Similarly, at any time, a lack of careful spectrum management can also lead to poor utilization. Careful channel allocation for 2.4 GHz interfaces can avoid inefficiencies in spectrum management for the first hop. Whereas, traffic engineering can help route traffic in the 5 GHz plane while minimizing interference. We discuss these challenges and techniques in more detail in the next section.


% \paragraphb{\farmernetes as a Service}
% The farmer may not need to buy and deploy this network themselves, this can be done by a service provider that brings in all the networking equipment along with robots and devices. They can deploy the networking equipment depending on the kind of tasks and stage of the canopy. It may host edge servers either in trucks parked near the farm or a building with a power supply near the farm.




==> workload-table.tex <==
\begin{table*}[!ht]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{|p{2.9cm}|p{6.55cm}|p{6.9cm}|}
         \multicolumn{3}{c}{  } \\
         \hline
         \textbf{Task} & \textbf{Bandwidth required}  & \textbf{Use-cases}  \\\hline
         Tele-operated robots & 5-10 Mbps \cite{latency_video, video_bitrates} & Remote tele-operation for assistance, \& virtual walkthroughs.\\\hline
         Edge-controlled robots & 10s of Mbps (requires high resolution images from multiple angles for accurate predictions) \cite{sivakumar2021visualnav, kamtikar2021fruitarm}  & Complex manipulation tasks (e.g. fruit picking, weeding, etc) \\\hline
         \multicolumn{3}{c}{\textbf{(a) Real-time operation} \vspace{-10pt}} \\ 
    \end{tabular}
    \begin{tabular}{|p{2.9cm}|p{4.7cm}|p{2.9cm}|p{5.5cm}|}
         \multicolumn{4}{c}{  } \\
         \hline
         \textbf{Sensor type}& \textbf{Data Volumes} & \textbf{Collection Frequency} & \textbf{Use-cases}  \\\hline
         RGB cameras & 25-100 MB per acre & multiple times a day  & Visual inputs for farmers\\\hline
         Thermal cameras & $\approx$15 MB per acre & multiple times a day & Assess water shortage and heat stress\\\hline
         Multi-spectral cameras & 500MB-2.5GB per acre & once a week & Plant health, yield, and disease prediction\\\hline
         \multicolumn{4}{c}{\textbf{(b) High-bandwidth data collection}} 
    \end{tabular}
    \caption{Examples of network tasks for precision agriculture. \radhika{move this table to appendix if desperate.}}
    \label{tab:network_tasks}\vspace{-0.1in}
\end{table*}

% \begin{table*}[!ht]
%     \centering
%     \footnotesize
%     \renewcommand{\arraystretch}{1.1}
%     \begin{tabular}{|p{2.9cm}|p{4.7cm}|p{2.9cm}|p{5.5cm}|}
%          \multicolumn{4}{c}{  } \\
%          \hline
%          \textbf{Task} & \multicolumn{2}{c}{\textbf{Bandwidth required}}  & \textbf{Use-cases}  \\\hline
%          Teleoperating robots/drones & \multicolumn{2}{p{7.5}}{5-10 Mbps \cite{latency_video, video_bitrates}}  & Remote tele-operation for assistance, \& virtual walkthroughs.\\\hline
%          Edge-controlled robots & \multicolumn{2}{p{7.5}}{10s of Mbps (requires high resolution images from multiple angles for accurate predictions)} \cite{sivakumar2021visualnav, kamtikar2021fruitarm}  & Complex manipulation tasks (e.g. fruit picking, weeding, etc) \\\hline
%          \multicolumn{4}{c}{\textbf{(a) Real-time operation}} \\ 
%          \multicolumn{4}{c}{  } \\
%          \hline
%          \textbf{Sensor type}& \textbf{Data Volumes} & \textbf{Collection Frequency} & \textbf{Use-cases}  \\\hline
%          RGB cameras & 50-200 MB per hectare & multiple times a day  & Visual inputs for farmers\\\hline
%          Thermal cameras & $\approx$30 MB per hectare & multiple times a day & Assess water shortage and heat stress\\\hline
%          Multi-spectral cameras & 1-5 GB per hectare & once a week & Plant health, yield, and disease prediction\\\hline
%          \multicolumn{4}{c}{\textbf{(b) High-bandwidth data collection}} 
%     \end{tabular}
%     \caption{Examples of network tasks for precision agriculture.\radhika{maybe remove the latency column in the table?}}
%     \label{tab:network_tasks}\vspace{-0.1in}
% \end{table*}


==> workloads-old.tex <==
\section{Workload}

Recent years have seen an increase in uptake of smart agriculture to keep up with high food demand. 
Such agriculture techniques are based on principle of precision agriculture, which argues for spatially and temporally targeted treatment of agriculture lands based on the observed data.
This not only help increase production, they also help reduce labour cost, decrease wastage, and improves sustainability. \radhika{repeated in intro, can perhaps cut (after moving some phrases to the intro)}
We surveyed 12 agronomists from 2 institutions regarding networking needs of their smart solutions. In addition, we also reviewed literature in this space to  characterize workloads of different precision agriculture applications \radhika{add cites}.

\subsection{Survey Takeaways}

Although many motivating applications already exist as we discuss in next section, another goal of surveying was to challenge the critical assumption of lack of high throughput when agronomists design smart farm solutions. The questionnaire for the survey asked questions related to the projects agronomists are working on, what kind of networking needs these solutions have? And additionally how a high throughput network would help deployability and innovation in smart agriculture research? Following are some key takeaways from the survey:

\begin{enumerate}
    \item Applications may collect diverse kinds of data including RGB, thermal and hyperspectral images, LIDAR, sensor data such as thermometer, pH, spectroradiometers, with RGB images being the most common (N= 11/12).
    \item In most cases, this data needs to be processed at some edge server (N=8/12) or on the collecting device itself (N=5/12). 
    \item For many cases (N=4/12), real time communication is required. Whereas in other cases, data needs to be processed in a few hours (N=3/12) or few days (N=3/12). 
    \item Despite the fact that most agronomists (N= 8/12) consider lack of high throughput network a critical assumption in their solution, most (N=7/12) require a network capable of being able to communicate RGB images and videos for their solutions to work.
    \item All participants (N=12/12) feel that a high throughput network will make it easier to deploy smart agriculture solutions and enable innovation in the space. 
\end{enumerate}

\subsection{Workload Characterization}

Below we discuss some classes of workload based on our survey and existing work. Some applications may require high throughput real time support from the network, while other applications may have a lot of data to send but may have deadlines in hours or days. However, all applications have flexibility in terms of when they are scheduled as we discuss with some motivating examples ahead.

\subsubsection{Real Time Tasks}

Many smart agriculture applications require real time support from the network, especially if they rely on edge server or some kind of human intervention. These include applications relying on complex classification or actuation tasks e.g. targeted bug spraying \cite{insect_detection}, fruit picking \cite{bogue2020fruit, kamtikar2021fruitarm, tang2020fruitrecognition}, teleoperation and visual navigation \cite{sivakumar2021visualnav}. Automating these tasks is important to address labour shortage \cite{bogue2020fruit} and improve crop health. These tasks pack a lot of complexity e.g. something as trivial as fruit picking requires the robot to be able to navigate narrow plant rows, identify ripe fruits and operate actuation arm. All of them are separate tasks requiring different machine learning models. These solutions may rely on different datastreams including RGB images from multiple cameras and may require network throughput between 5-20 Mbps. While real time nature of these tasks is apparent, it should be noted that these tasks still have flexibility in terms of when they need to be started. For example, fruit picking in a particular row can be started a few minutes later. Moreover, while a task like fruit picking can easily be paused to distribute resources elsewhere for a higher priority task, preempting bug spraying is not possible. So while all tasks have flexibility in terms of scheduling, some tasks may additionally allow flexibility of preemption.

Other real time applications include mechanical weeding, under canopy cover crop planting and other plant manipulation tasks.

\subsubsection{Tasks with Pseudo Deadlines}

Such tasks may need to be performed daily or even weekly but usually just involve some kind of data collection. For a number of precision agriculture applications like precision irrigation, targeted fertilizers, data needs to be collected from the farm periodically. For example, thermal imaging and/or sensor data may need to be collected multiple times a day to determine moisture contents to determine when and how much to irrigate different parts of farm. Hyperspectral imaging may need to be done every now and then to determine plant health. Similarly, a number of other sensors produce different kinds of data for different applications e.g. pH sensors to aid with precision fertilizing, thermometers etc. Similarly, for a lot of phenotyping research, a lot of data needs to be collected in a certain window of time.
All this data can add up e.g. hyperspectral imaging of 1 hectare produces 1.5 GB of data. Thus collecting this data can be challenging despite having flexible deadlines.\radhika{try to add cites}

\subsubsection{Tasks with No Deadline}

Some other data collection may not have any explicit deadline e.g. data to send to cloud for statistics and modeling etc.
